Deep Prior Learning for Embodied Perception

Embodied systems need geometric perception that exploits available observations beyond images alone. Recent feed-forward 3D models incorporate geometric priors, including camera poses, intrinsics, and depth. However, handling noisy poses, preserving accurate priors, and recovering physical scale require more than simply accepting these inputs. We introduce \emph{Vision-Prior Geometry Grounded Transformer} (VPGGT), a VGGT-based framework that extends OmniVGGT for prior-aware embodied perception. We formulate sensor-motivated pose corruptions from ground-truth trajectories for training and introduce a parameter-free \emph{prior residual connection} (PRC) to mitigate \emph{prior dilution}, where predictions are less accurate than their supplied pose priors. Our noise formulation targets camera poses; supplied intrinsics and depth receive no additional corruption. We further introduce \emph{Metric Global Attention}, which conditions a global scale token on available pose and depth scales and predicts a shared metric scaling factor for the geometric outputs. Experiments across four datasets show that \emph{PRC} improves translation-direction accuracy and joint pose AUC over a matched training baseline when camera priors are provided for all views, under both exact and corrupted poses. These results support explicit prior access during refinement as a useful addition to feature-level conditioning.

==> tables/generated/main_auxiliary.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation of auxiliary information guidance.} Depth and pose results on held-out TUM RGB-D and C3VD sequences. Parentheses show signed gains over matched OmniVGGT-FT inputs for PRC-only results, with positive gains in blue. Green, when available, compares released OmniVGGT with VGGT in the RGB-only setting. Depth is median-aligned per frame; RTA and AUC are sign-free.}
\label{tab:auxiliary_guidance}
\begin{minipage}[t]{0.49\linewidth}
\centering
{\scriptsize\textbf{(a) TUM RGB-D}\par}
\input{tables/generated/main_tum-eval.tex}
\end{minipage}\hfill
\begin{minipage}[t]{0.49\linewidth}
\centering
{\scriptsize\textbf{(b) C3VD}\par}
\input{tables/generated/main_c3vd-eval.tex}
\end{minipage}
\par\smallskip
{\scriptsize D/C: provided-view percentages; GT/N: exact/noisy camera poses; FT: matched fine-tuning. Bold marks matched-pair wins. All angular thresholds are in degrees. NR denotes an unavailable result.\par}
\end{table}


==> tables/generated/main_c3vd-eval.tex <==
\begingroup\scriptsize
\setlength{\tabcolsep}{0.8pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}rrcrrrrr@{}}
\toprule
\multicolumn{3}{c}{Priors} & \multicolumn{2}{c}{Depth} & \multicolumn{3}{c}{Camera} \\
\cmidrule(lr){1-3}\cmidrule(lr){4-5}\cmidrule(l){6-8}
D & C & Pose & AbsRel$\downarrow$ & $\delta_1\uparrow$ & RRA@5$\uparrow$ & RTA@5$\uparrow$ & AUC@30$\uparrow$ \\
\midrule
\multicolumn{8}{l}{\textbf{Input camera-prior reference}} \\
0 & 100 & GT & -- & -- & 100.00 & 100.00 & 100.00 \\
0 & 100 & N & -- & -- & 100.00 & 57.73 & 71.73 \\
\midrule
\multicolumn{8}{l}{\textbf{VGGT, released}} \\
0 & 0 & -- & \textcolor{gray}{NR} & \textcolor{gray}{NR} & \textcolor{gray}{NR} & \textcolor{gray}{NR} & \textcolor{gray}{NR} \\
\midrule
\multicolumn{8}{l}{\textbf{OmniVGGT, released}} \\
0 & 0 & -- & 0.511 & 29.89 & 87.51 & 14.67 & 40.88 \\
100 & 100 & GT & 0.036 & 98.57 & 100.00 & 45.88 & 64.70 \\
100 & 100 & N & 0.036 & 98.57 & 100.00 & 39.56 & 57.23 \\
\midrule
\multicolumn{8}{l}{\textbf{OmniVGGT-FT}} \\
0 & 0 & -- & 0.055 & 97.87 & 100.00 & \textbf{29.19} & \textbf{61.55} \\
0 & 100 & GT & 0.055 & 97.90 & 100.00 & 43.16 & 69.42 \\
0 & 100 & N & 0.055 & 97.90 & 100.00 & 42.62 & 67.73 \\
100 & 100 & GT & 0.004 & 99.98 & 100.00 & 55.51 & 76.36 \\
100 & 100 & N & 0.004 & 99.98 & 100.00 & 54.07 & \textbf{74.80} \\
\midrule
\multicolumn{8}{l}{\textbf{VPGGT, PRC only}} \\
0 & 0 & -- & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.09}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{27.75\\(-1.43)} & \shortstack[r]{61.49\\(-0.07)} \\
\cmidrule(l){1-8}
30 & 0 & -- & \shortstack[r]{0.015\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{99.80}\\\textcolor{prcBlue}{(+0.02)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{26.12}\\\textcolor{prcBlue}{(+0.79)}} & \shortstack[r]{\textbf{54.92}\\\textcolor{prcBlue}{(+0.24)}} \\
50 & 0 & -- & \shortstack[r]{\textbf{0.010}\\(0.000)} & \shortstack[r]{\textbf{99.87}\\(0.00)} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{30.72}\\\textcolor{prcBlue}{(+0.20)}} & \shortstack[r]{\textbf{57.29}\\\textcolor{prcBlue}{(+0.29)}} \\
70 & 0 & -- & \shortstack[r]{0.007\\(0.000)} & \shortstack[r]{99.92\\(0.00)} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{36.99\\(-0.49)} & \shortstack[r]{\textbf{62.33}\\\textcolor{prcBlue}{(+0.09)}} \\
100 & 0 & -- & \shortstack[r]{0.004\\(0.000)} & \shortstack[r]{99.98\\(0.00)} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{54.22}\\\textcolor{prcBlue}{(+0.99)}} & \shortstack[r]{\textbf{74.59}\\\textcolor{prcBlue}{(+0.33)}} \\
\cmidrule(l){1-8}
0 & 30 & GT & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.10}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{28.74}\\\textcolor{prcBlue}{(+0.79)}} & \shortstack[r]{\textbf{60.89}\\\textcolor{prcBlue}{(+0.46)}} \\
0 & 50 & GT & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.11}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{35.26}\\\textcolor{prcBlue}{(+6.37)}} & \shortstack[r]{\textbf{64.52}\\\textcolor{prcBlue}{(+2.68)}} \\
0 & 70 & GT & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.11}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{46.81}\\\textcolor{prcBlue}{(+14.52)}} & \shortstack[r]{\textbf{71.01}\\\textcolor{prcBlue}{(+6.51)}} \\
0 & 100 & GT & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.11}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{76.74}\\\textcolor{prcBlue}{(+33.58)}} & \shortstack[r]{\textbf{88.48}\\\textcolor{prcBlue}{(+19.06)}} \\
\cmidrule(l){1-8}
0 & 30 & N & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.10}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{26.02\\(-1.63)} & \shortstack[r]{58.60\\(-1.02)} \\
0 & 50 & N & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.11}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{28.84}\\\textcolor{prcBlue}{(+0.84)}} & \shortstack[r]{58.77\\(-1.62)} \\
0 & 70 & N & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.11}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{34.77}\\\textcolor{prcBlue}{(+2.91)}} & \shortstack[r]{61.50\\(-1.44)} \\
0 & 100 & N & \shortstack[r]{0.055\\\textcolor{prcBlue}{(+0.001)}} & \shortstack[r]{\textbf{98.11}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{55.46}\\\textcolor{prcBlue}{(+12.84)}} & \shortstack[r]{\textbf{72.81}\\\textcolor{prcBlue}{(+5.08)}} \\
\cmidrule(l){1-8}
100 & 100 & GT & \shortstack[r]{0.004\\(0.000)} & \shortstack[r]{99.98\\(0.00)} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{81.78}\\\textcolor{prcBlue}{(+26.27)}} & \shortstack[r]{\textbf{91.04}\\\textcolor{prcBlue}{(+14.67)}} \\
100 & 100 & N & \shortstack[r]{0.004\\(0.000)} & \shortstack[r]{99.98\\(0.00)} & \shortstack[r]{100.00\\(0.00)} & \shortstack[r]{\textbf{60.40}\\\textcolor{prcBlue}{(+6.32)}} & \shortstack[r]{74.53\\(-0.27)} \\
\bottomrule
\end{tabular*}
\endgroup


==> tables/generated/main_tum-eval.tex <==
\begingroup\scriptsize
\setlength{\tabcolsep}{0.8pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}rrcrrrrr@{}}
\toprule
\multicolumn{3}{c}{Priors} & \multicolumn{2}{c}{Depth} & \multicolumn{3}{c}{Camera} \\
\cmidrule(lr){1-3}\cmidrule(lr){4-5}\cmidrule(l){6-8}
D & C & Pose & AbsRel$\downarrow$ & $\delta_1\uparrow$ & RRA@5$\uparrow$ & RTA@5$\uparrow$ & AUC@30$\uparrow$ \\
\midrule
\multicolumn{8}{l}{\textbf{Input camera-prior reference}} \\
0 & 100 & GT & -- & -- & 100.00 & 100.00 & 100.00 \\
0 & 100 & N & -- & -- & 100.00 & 66.00 & 81.07 \\
\midrule
\multicolumn{8}{l}{\textbf{VGGT, released}} \\
0 & 0 & -- & \textcolor{gray}{NR} & \textcolor{gray}{NR} & \textcolor{gray}{NR} & \textcolor{gray}{NR} & \textcolor{gray}{NR} \\
\midrule
\multicolumn{8}{l}{\textbf{OmniVGGT, released}} \\
0 & 0 & -- & 0.078 & 92.57 & 99.67 & 38.00 & 61.94 \\
100 & 100 & GT & 0.018 & 99.20 & 97.22 & 67.78 & 76.66 \\
100 & 100 & N & 0.018 & 99.20 & 97.22 & 57.11 & 71.30 \\
\midrule
\multicolumn{8}{l}{\textbf{OmniVGGT-FT}} \\
0 & 0 & -- & 0.058 & \textbf{94.64} & 96.33 & \textbf{51.22} & 69.17 \\
0 & 100 & GT & \textbf{0.057} & \textbf{94.69} & \textbf{97.22} & 58.78 & 71.04 \\
0 & 100 & N & \textbf{0.057} & \textbf{94.70} & 97.22 & 58.89 & 70.89 \\
100 & 100 & GT & 0.009 & 99.76 & 95.44 & 55.89 & 71.86 \\
100 & 100 & N & 0.009 & 99.76 & 95.44 & 55.56 & 71.16 \\
\midrule
\multicolumn{8}{l}{\textbf{VPGGT, PRC only}} \\
0 & 0 & -- & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.41\\(-0.23)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+0.89)}} & \shortstack[r]{50.33\\(-0.89)} & \shortstack[r]{\textbf{69.33}\\\textcolor{prcBlue}{(+0.16)}} \\
\cmidrule(l){1-8}
30 & 0 & -- & \shortstack[r]{0.031\\(0.000)} & \shortstack[r]{98.04\\(-0.01)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+0.22)}} & \shortstack[r]{\textbf{48.56}\\\textcolor{prcBlue}{(+1.22)}} & \shortstack[r]{\textbf{66.66}\\\textcolor{prcBlue}{(+0.20)}} \\
50 & 0 & -- & \shortstack[r]{\textbf{0.023}\\(0.000)} & \shortstack[r]{98.57\\(0.00)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+1.67)}} & \shortstack[r]{\textbf{45.89}\\\textcolor{prcBlue}{(+0.11)}} & \shortstack[r]{\textbf{66.46}\\\textcolor{prcBlue}{(+0.25)}} \\
70 & 0 & -- & \shortstack[r]{\textbf{0.016}\\(0.000)} & \shortstack[r]{99.11\\(0.00)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+1.89)}} & \shortstack[r]{\textbf{49.22}\\\textcolor{prcBlue}{(+1.33)}} & \shortstack[r]{\textbf{68.87}\\\textcolor{prcBlue}{(+0.65)}} \\
100 & 0 & -- & \shortstack[r]{0.009\\(0.000)} & \shortstack[r]{99.76\\(0.00)} & \shortstack[r]{\textbf{96.22}\\\textcolor{prcBlue}{(+0.78)}} & \shortstack[r]{\textbf{52.33}\\\textcolor{prcBlue}{(+0.44)}} & \shortstack[r]{\textbf{71.77}\\\textcolor{prcBlue}{(+1.06)}} \\
\cmidrule(l){1-8}
0 & 30 & GT & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.44\\(-0.22)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+0.78)}} & \shortstack[r]{\textbf{51.00}\\\textcolor{prcBlue}{(+2.00)}} & \shortstack[r]{\textbf{69.29}\\\textcolor{prcBlue}{(+1.37)}} \\
0 & 50 & GT & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.46\\(-0.22)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+0.78)}} & \shortstack[r]{\textbf{55.00}\\\textcolor{prcBlue}{(+5.33)}} & \shortstack[r]{\textbf{70.74}\\\textcolor{prcBlue}{(+3.56)}} \\
0 & 70 & GT & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.46\\(-0.23)} & \shortstack[r]{\textbf{96.56}\\\textcolor{prcBlue}{(+0.44)}} & \shortstack[r]{\textbf{60.11}\\\textcolor{prcBlue}{(+8.56)}} & \shortstack[r]{\textbf{73.50}\\\textcolor{prcBlue}{(+5.24)}} \\
0 & 100 & GT & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.49\\(-0.20)} & \shortstack[r]{96.89\\(-0.33)} & \shortstack[r]{\textbf{73.78}\\\textcolor{prcBlue}{(+15.00)}} & \shortstack[r]{\textbf{80.46}\\\textcolor{prcBlue}{(+9.42)}} \\
\cmidrule(l){1-8}
0 & 30 & N & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.44\\(-0.22)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+0.78)}} & \shortstack[r]{\textbf{49.78}\\\textcolor{prcBlue}{(+0.56)}} & \shortstack[r]{\textbf{68.64}\\\textcolor{prcBlue}{(+0.79)}} \\
0 & 50 & N & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.46\\(-0.22)} & \shortstack[r]{\textbf{97.22}\\\textcolor{prcBlue}{(+0.78)}} & \shortstack[r]{\textbf{51.11}\\\textcolor{prcBlue}{(+2.00)}} & \shortstack[r]{\textbf{69.28}\\\textcolor{prcBlue}{(+2.28)}} \\
0 & 70 & N & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.46\\(-0.23)} & \shortstack[r]{\textbf{96.56}\\\textcolor{prcBlue}{(+0.44)}} & \shortstack[r]{\textbf{55.00}\\\textcolor{prcBlue}{(+3.56)}} & \shortstack[r]{\textbf{70.89}\\\textcolor{prcBlue}{(+2.64)}} \\
0 & 100 & N & \shortstack[r]{0.058\\(-0.001)} & \shortstack[r]{94.51\\(-0.19)} & \shortstack[r]{97.22\\(0.00)} & \shortstack[r]{\textbf{67.00}\\\textcolor{prcBlue}{(+8.11)}} & \shortstack[r]{\textbf{76.37}\\\textcolor{prcBlue}{(+5.48)}} \\
\cmidrule(l){1-8}
100 & 100 & GT & \shortstack[r]{0.009\\(0.000)} & \shortstack[r]{99.76\\(0.00)} & \shortstack[r]{\textbf{96.56}\\\textcolor{prcBlue}{(+1.11)}} & \shortstack[r]{\textbf{68.44}\\\textcolor{prcBlue}{(+12.56)}} & \shortstack[r]{\textbf{79.08}\\\textcolor{prcBlue}{(+7.22)}} \\
100 & 100 & N & \shortstack[r]{0.009\\(0.000)} & \shortstack[r]{99.76\\(0.00)} & \shortstack[r]{\textbf{96.67}\\\textcolor{prcBlue}{(+1.22)}} & \shortstack[r]{\textbf{63.44}\\\textcolor{prcBlue}{(+7.89)}} & \shortstack[r]{\textbf{75.31}\\\textcolor{prcBlue}{(+4.15)}} \\
\bottomrule
\end{tabular*}
\endgroup


==> tables/generated/released_c3vd-eval_depth.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, released-weight intervention. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:released-c3vd-eval-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & A0 & 0.511 & 29.89 & 0.511 & 29.89 & 1.96e-04 & 450 & 450 \\
0 & 0 & -- & A1 & 0.511 & 29.89 & 0.511 & 29.89 & 1.96e-04 & 450 & 450 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 0.080 & 92.61 & 0.097 & 90.05 & 3.44e-04 & 450 & 315 \\
30 & 0 & -- & A1 & 0.080 & 92.61 & 0.097 & 90.05 & 3.44e-04 & 450 & 315 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 0.060 & 95.65 & 0.079 & 92.81 & 4.50e-04 & 450 & 225 \\
50 & 0 & -- & A1 & 0.060 & 95.65 & 0.079 & 92.81 & 4.50e-04 & 450 & 225 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 0.048 & 97.35 & 0.066 & 94.83 & 4.87e-04 & 450 & 135 \\
70 & 0 & -- & A1 & 0.048 & 97.35 & 0.066 & 94.83 & 4.87e-04 & 450 & 135 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 0.039 & 98.49 & -- & -- & 1.35e-04 & 450 & 0 \\
100 & 0 & -- & A1 & 0.039 & 98.49 & -- & -- & 1.35e-04 & 450 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 0.500 & 30.43 & 0.500 & 30.43 & 3.56e-04 & 450 & 450 \\
0 & 30 & GT & A1 & 0.500 & 30.43 & 0.500 & 30.43 & \textbf{3.20e-04} & 450 & 450 \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 0.497 & 30.57 & 0.497 & 30.57 & 3.62e-04 & 450 & 450 \\
0 & 50 & GT & A1 & 0.497 & 30.57 & 0.497 & 30.57 & \textbf{3.35e-04} & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 0.493 & 30.70 & 0.493 & 30.70 & 4.18e-04 & 450 & 450 \\
0 & 70 & GT & A1 & 0.493 & 30.70 & 0.493 & 30.70 & \textbf{3.97e-04} & 450 & 450 \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 0.485 & 30.96 & 0.485 & 30.96 & 7.69e-05 & 450 & 450 \\
0 & 100 & GT & A1 & 0.485 & 30.96 & 0.485 & 30.96 & \textbf{7.00e-05} & 450 & 450 \\
\addlinespace[1pt]
0 & 30 & N & A0 & 0.500 & 30.44 & 0.500 & 30.44 & 3.55e-04 & 450 & 450 \\
0 & 30 & N & A1 & 0.500 & 30.44 & 0.500 & 30.44 & \textbf{3.20e-04} & 450 & 450 \\
\addlinespace[1pt]
0 & 50 & N & A0 & 0.497 & 30.59 & 0.497 & 30.59 & 3.62e-04 & 450 & 450 \\
0 & 50 & N & A1 & 0.497 & 30.59 & 0.497 & 30.59 & \textbf{3.36e-04} & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & N & A0 & 0.493 & 30.72 & 0.493 & 30.72 & 4.17e-04 & 450 & 450 \\
0 & 70 & N & A1 & 0.493 & 30.72 & 0.493 & 30.72 & \textbf{3.98e-04} & 450 & 450 \\
\addlinespace[1pt]
0 & 100 & N & A0 & 0.485 & 30.95 & 0.485 & 30.95 & \textbf{8.73e-05} & 450 & 450 \\
0 & 100 & N & A1 & 0.485 & 30.95 & 0.485 & 30.95 & 8.75e-05 & 450 & 450 \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 0.036 & 98.57 & -- & -- & 1.09e-04 & 450 & 0 \\
100 & 100 & GT & A1 & 0.036 & 98.57 & -- & -- & \textbf{9.71e-05} & 450 & 0 \\
\addlinespace[1pt]
100 & 100 & N & A0 & 0.036 & 98.57 & -- & -- & 1.20e-04 & 450 & 0 \\
100 & 100 & N & A1 & 0.036 & 98.57 & -- & -- & \textbf{1.12e-04} & 450 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_c3vd-eval_directed.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, released-weight intervention. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:released-c3vd-eval-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 3.90 & 14.67 & 45.43 & 22.96 & 40.77 \\
0 & 0 & -- & A1 & 3.90 & 14.67 & 45.43 & 22.96 & 40.77 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 2.22 & 9.88 & 27.21 & 14.94 & 26.59 \\
30 & 0 & -- & A1 & 2.22 & 9.88 & 27.21 & 14.94 & 26.59 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 2.62 & 10.91 & 30.07 & 16.94 & 28.81 \\
50 & 0 & -- & A1 & 2.62 & 10.91 & 30.07 & 16.94 & 28.81 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 3.70 & 15.26 & 32.20 & 20.16 & 31.13 \\
70 & 0 & -- & A1 & 3.70 & 15.26 & 32.20 & 20.16 & 31.13 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 5.23 & 21.73 & 40.30 & 26.99 & 38.32 \\
100 & 0 & -- & A1 & 5.23 & 21.73 & 40.30 & 26.99 & 38.32 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 1.09 & \textbf{6.42} & 38.17 & 17.19 & 33.05 \\
0 & 30 & GT & A1 & \textbf{1.23} & 6.17 & \textbf{39.41} & \textbf{17.43} & \textbf{34.00} \\
\addlinespace[1pt]
0 & 50 & GT & A0 & \textbf{2.37} & \textbf{10.91} & \textbf{42.27} & \textbf{20.99} & \textbf{36.43} \\
0 & 50 & GT & A1 & 2.27 & 9.14 & 41.48 & 19.96 & 35.97 \\
\addlinespace[1pt]
0 & 70 & GT & A0 & \textbf{5.78} & \textbf{19.90} & \textbf{52.30} & \textbf{30.14} & \textbf{45.30} \\
0 & 70 & GT & A1 & 5.09 & 16.10 & 50.22 & 26.96 & 43.34 \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 13.78 & \textbf{45.23} & \textbf{80.69} & \textbf{55.83} & \textbf{70.48} \\
0 & 100 & GT & A1 & \textbf{15.01} & 42.27 & 77.58 & 52.45 & 68.19 \\
\addlinespace[1pt]
0 & 30 & N & A0 & \textbf{1.14} & 5.78 & 36.79 & 16.45 & 32.22 \\
0 & 30 & N & A1 & 1.04 & \textbf{5.88} & \textbf{37.83} & \textbf{16.49} & \textbf{32.80} \\
\addlinespace[1pt]
0 & 50 & N & A0 & \textbf{1.58} & \textbf{8.59} & \textbf{39.21} & \textbf{18.68} & \textbf{34.27} \\
0 & 50 & N & A1 & 1.43 & 7.65 & 38.17 & 17.78 & 33.62 \\
\addlinespace[1pt]
0 & 70 & N & A0 & \textbf{4.20} & \textbf{15.51} & \textbf{46.57} & \textbf{25.69} & \textbf{40.97} \\
0 & 70 & N & A1 & 4.05 & 12.79 & 44.10 & 22.76 & 38.81 \\
\addlinespace[1pt]
0 & 100 & N & A0 & \textbf{12.64} & \textbf{36.35} & \textbf{68.59} & \textbf{45.95} & \textbf{60.73} \\
0 & 100 & N & A1 & 12.44 & 35.65 & 66.02 & 44.42 & 59.03 \\
\addlinespace[1pt]
100 & 100 & GT & A0 & \textbf{24.94} & \textbf{45.88} & \textbf{70.57} & \textbf{50.43} & \textbf{64.18} \\
100 & 100 & GT & A1 & 15.16 & 37.33 & 58.27 & 41.24 & 55.01 \\
\addlinespace[1pt]
100 & 100 & N & A0 & \textbf{19.95} & \textbf{39.51} & \textbf{61.68} & \textbf{44.36} & \textbf{56.87} \\
100 & 100 & N & A1 & 13.04 & 32.10 & 53.28 & 37.15 & 50.37 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_c3vd-eval_pose.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, released-weight intervention. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:released-c3vd-eval-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 72.49 & 87.51 & 98.27 & 3.90 & 14.67 & 45.48 & 22.97 & 40.88 \\
0 & 0 & -- & A1 & 72.49 & 87.51 & 98.27 & 3.90 & 14.67 & 45.48 & 22.97 & 40.88 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 96.10 & 99.85 & 100.00 & 2.22 & 9.88 & 28.20 & 15.26 & 27.78 \\
30 & 0 & -- & A1 & 96.10 & 99.85 & 100.00 & 2.22 & 9.88 & 28.20 & 15.26 & 27.78 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 96.25 & 99.90 & 100.00 & 2.62 & 10.91 & 30.67 & 17.12 & 29.89 \\
50 & 0 & -- & A1 & 96.25 & 99.90 & 100.00 & 2.62 & 10.91 & 30.67 & 17.12 & 29.89 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 96.74 & 100.00 & 100.00 & 3.70 & 15.51 & 33.33 & 20.61 & 32.43 \\
70 & 0 & -- & A1 & 96.74 & 100.00 & 100.00 & 3.70 & 15.51 & 33.33 & 20.61 & 32.43 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 98.81 & 100.00 & 100.00 & 5.23 & 21.73 & 40.35 & 27.01 & 38.58 \\
100 & 0 & -- & A1 & 98.81 & 100.00 & 100.00 & 5.23 & 21.73 & 40.35 & 27.01 & 38.58 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & \textbf{71.36} & \textbf{89.43} & \textbf{98.77} & 1.14 & \textbf{6.62} & 38.91 & 17.50 & 34.27 \\
0 & 30 & GT & A1 & 67.36 & 89.04 & 98.52 & \textbf{1.23} & 6.37 & \textbf{40.49} & \textbf{17.90} & \textbf{35.06} \\
\addlinespace[1pt]
0 & 50 & GT & A0 & \textbf{70.27} & \textbf{88.54} & \textbf{98.32} & \textbf{2.37} & \textbf{11.01} & \textbf{43.26} & \textbf{21.31} & \textbf{37.56} \\
0 & 50 & GT & A1 & 65.98 & 87.95 & 97.93 & 2.27 & 9.28 & 42.12 & 20.20 & 36.66 \\
\addlinespace[1pt]
0 & 70 & GT & A0 & \textbf{74.02} & \textbf{89.93} & \textbf{98.17} & \textbf{5.78} & \textbf{19.95} & \textbf{53.63} & \textbf{30.65} & \textbf{46.98} \\
0 & 70 & GT & A1 & 72.59 & 89.14 & 97.68 & 5.19 & 16.44 & 51.80 & 27.73 & 44.99 \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 91.56 & 98.62 & 100.00 & 13.78 & \textbf{45.23} & \textbf{81.43} & \textbf{56.05} & \textbf{71.44} \\
0 & 100 & GT & A1 & \textbf{97.23} & \textbf{100.00} & 100.00 & \textbf{15.01} & 42.42 & 78.81 & 52.86 & 69.54 \\
\addlinespace[1pt]
0 & 30 & N & A0 & \textbf{71.41} & \textbf{89.48} & \textbf{98.77} & \textbf{1.14} & 5.93 & 37.53 & 16.70 & 33.41 \\
0 & 30 & N & A1 & 67.80 & 89.04 & 98.52 & 1.04 & 5.93 & \textbf{38.37} & \textbf{16.73} & \textbf{33.63} \\
\addlinespace[1pt]
0 & 50 & N & A0 & \textbf{70.12} & \textbf{88.64} & \textbf{98.32} & \textbf{1.58} & \textbf{8.59} & \textbf{39.65} & \textbf{18.80} & \textbf{35.08} \\
0 & 50 & N & A1 & 66.27 & 88.10 & 97.93 & 1.43 & 7.70 & 38.52 & 17.88 & 34.08 \\
\addlinespace[1pt]
0 & 70 & N & A0 & \textbf{73.93} & \textbf{89.98} & \textbf{98.17} & \textbf{4.20} & \textbf{15.56} & \textbf{47.36} & \textbf{25.90} & \textbf{42.08} \\
0 & 70 & N & A1 & 72.69 & 89.19 & 97.68 & 4.05 & 12.79 & 44.79 & 22.99 & 39.74 \\
\addlinespace[1pt]
0 & 100 & N & A0 & 91.56 & 98.67 & 100.00 & \textbf{12.64} & \textbf{36.35} & \textbf{68.69} & \textbf{45.99} & \textbf{61.05} \\
0 & 100 & N & A1 & \textbf{97.28} & \textbf{100.00} & 100.00 & 12.44 & 35.70 & 66.27 & 44.51 & 59.49 \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 100.00 & 100.00 & 100.00 & \textbf{24.94} & \textbf{45.88} & \textbf{70.96} & \textbf{50.52} & \textbf{64.70} \\
100 & 100 & GT & A1 & 100.00 & 100.00 & 100.00 & 15.16 & 37.38 & 59.16 & 41.53 & 56.00 \\
\addlinespace[1pt]
100 & 100 & N & A0 & 100.00 & 100.00 & 100.00 & \textbf{19.95} & \textbf{39.56} & \textbf{61.83} & \textbf{44.43} & \textbf{57.23} \\
100 & 100 & N & A1 & 100.00 & 100.00 & 100.00 & 13.04 & 32.10 & 53.43 & 37.19 & 50.67 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_c3vd-eval_retention.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:released-c3vd-eval-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 135 & 135 \\
0 & 30 & GT & A0 & 100.00 & 100.00 & 2.22 & 15.56 & 29.04 & 45.95 & 135 & 135 \\
0 & 30 & GT & A1 & 100.00 & 100.00 & 2.96 & 11.11 & 27.21 & 46.74 & 135 & 135 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 450 & 450 \\
0 & 50 & GT & A0 & 97.78 & 100.00 & 6.67 & 30.00 & 39.76 & 57.51 & 450 & 450 \\
0 & 50 & GT & A1 & 99.78 & 100.00 & 6.44 & 22.44 & 34.25 & 52.33 & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 945 & 945 \\
0 & 70 & GT & A0 & 94.71 & 100.00 & 11.64 & 38.62 & 48.57 & 64.87 & 945 & 945 \\
0 & 70 & GT & A1 & 98.84 & 100.00 & 9.84 & 30.69 & 42.38 & 60.13 & 945 & 945 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 2025 & 2025 \\
0 & 100 & GT & A0 & 91.56 & 98.62 & 13.78 & 45.23 & 56.05 & 71.44 & 2025 & 2025 \\
0 & 100 & GT & A1 & 97.23 & 100.00 & 15.01 & 42.42 & 52.86 & 69.54 & 2025 & 2025 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 17.04 & 43.70 & 47.85 & 59.43 & 135 & 135 \\
0 & 30 & N & A0 & 100.00 & 100.00 & 1.48 & 9.63 & 21.68 & 36.52 & 135 & 135 \\
0 & 30 & N & A1 & 100.00 & 100.00 & 1.48 & 10.37 & 19.90 & 35.01 & 135 & 135 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 26.67 & 49.78 & 52.47 & 63.66 & 450 & 450 \\
0 & 50 & N & A0 & 97.56 & 100.00 & 3.78 & 21.78 & 31.20 & 48.13 & 450 & 450 \\
0 & 50 & N & A1 & 99.78 & 100.00 & 3.11 & 17.33 & 27.24 & 43.03 & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 31.43 & 52.80 & 56.59 & 67.76 & 945 & 945 \\
0 & 70 & N & A0 & 94.71 & 100.00 & 8.47 & 29.74 & 39.29 & 54.91 & 945 & 945 \\
0 & 70 & N & A1 & 98.73 & 100.00 & 7.83 & 23.70 & 33.52 & 49.76 & 945 & 945 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 100.00 & 100.00 & 37.28 & 57.73 & 61.36 & 71.73 & 2025 & 2025 \\
0 & 100 & N & A0 & 91.56 & 98.67 & 12.64 & 36.35 & 45.99 & 61.05 & 2025 & 2025 \\
0 & 100 & N & A1 & 97.28 & 100.00 & 12.44 & 35.70 & 44.51 & 59.49 & 2025 & 2025 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 2025 & 2025 \\
100 & 100 & GT & A0 & 100.00 & 100.00 & 24.94 & 45.88 & 50.52 & 64.70 & 2025 & 2025 \\
100 & 100 & GT & A1 & 100.00 & 100.00 & 15.16 & 37.38 & 41.53 & 56.00 & 2025 & 2025 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 100.00 & 100.00 & 37.28 & 57.73 & 61.36 & 71.73 & 2025 & 2025 \\
100 & 100 & N & A0 & 100.00 & 100.00 & 19.95 & 39.56 & 44.43 & 57.23 & 2025 & 2025 \\
100 & 100 & N & A1 & 100.00 & 100.00 & 13.04 & 32.10 & 37.19 & 50.67 & 2025 & 2025 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_tum-eval_depth.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, released-weight intervention. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:released-tum-eval-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & A0 & 0.078 & 92.57 & 0.078 & 92.57 & 5.54e-03 & 200 & 200 \\
0 & 0 & -- & A1 & 0.078 & 92.57 & 0.078 & 92.57 & 5.54e-03 & 200 & 200 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 0.044 & 96.66 & 0.053 & 95.75 & 5.96e-03 & 200 & 140 \\
30 & 0 & -- & A1 & 0.044 & 96.66 & 0.053 & 95.75 & 5.96e-03 & 200 & 140 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 0.036 & 97.48 & 0.052 & 96.02 & 5.57e-03 & 200 & 100 \\
50 & 0 & -- & A1 & 0.036 & 97.48 & 0.052 & 96.02 & 5.57e-03 & 200 & 100 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 0.028 & 98.19 & 0.049 & 96.24 & 5.37e-03 & 200 & 60 \\
70 & 0 & -- & A1 & 0.028 & 98.19 & 0.049 & 96.24 & 5.37e-03 & 200 & 60 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 0.018 & 99.20 & -- & -- & 5.42e-03 & 200 & 0 \\
100 & 0 & -- & A1 & 0.018 & 99.20 & -- & -- & 5.42e-03 & 200 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 0.077 & 92.63 & 0.077 & 92.63 & 6.23e-03 & 200 & 200 \\
0 & 30 & GT & A1 & 0.077 & 92.63 & 0.077 & 92.63 & \textbf{6.02e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 0.078 & 92.42 & 0.078 & 92.42 & 6.19e-03 & 200 & 200 \\
0 & 50 & GT & A1 & 0.078 & 92.42 & 0.078 & 92.42 & \textbf{6.12e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 0.078 & 92.37 & 0.078 & 92.37 & \textbf{6.00e-03} & 200 & 200 \\
0 & 70 & GT & A1 & 0.078 & 92.37 & 0.078 & 92.37 & 6.07e-03 & 200 & 200 \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 0.078 & 92.18 & 0.078 & 92.18 & \textbf{2.43e-03} & 200 & 200 \\
0 & 100 & GT & A1 & 0.078 & 92.18 & 0.078 & 92.18 & 2.51e-03 & 200 & 200 \\
\addlinespace[1pt]
0 & 30 & N & A0 & 0.077 & 92.63 & 0.077 & 92.63 & 6.34e-03 & 200 & 200 \\
0 & 30 & N & A1 & 0.077 & 92.63 & 0.077 & 92.63 & \textbf{6.12e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 50 & N & A0 & 0.078 & 92.43 & 0.078 & 92.43 & 6.48e-03 & 200 & 200 \\
0 & 50 & N & A1 & 0.078 & 92.43 & 0.078 & 92.43 & \textbf{6.39e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & N & A0 & 0.078 & 92.35 & 0.078 & 92.35 & \textbf{6.29e-03} & 200 & 200 \\
0 & 70 & N & A1 & 0.078 & 92.35 & 0.078 & 92.35 & 6.41e-03 & 200 & 200 \\
\addlinespace[1pt]
0 & 100 & N & A0 & 0.078 & 92.23 & 0.078 & 92.23 & \textbf{2.63e-03} & 200 & 200 \\
0 & 100 & N & A1 & 0.078 & 92.23 & 0.078 & 92.23 & 2.76e-03 & 200 & 200 \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 0.018 & 99.20 & -- & -- & 2.81e-03 & 200 & 0 \\
100 & 100 & GT & A1 & 0.018 & 99.20 & -- & -- & \textbf{2.58e-03} & 200 & 0 \\
\addlinespace[1pt]
100 & 100 & N & A0 & 0.018 & 99.20 & -- & -- & 2.95e-03 & 200 & 0 \\
100 & 100 & N & A1 & 0.018 & 99.20 & -- & -- & \textbf{2.73e-03} & 200 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_tum-eval_directed.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, released-weight intervention. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:released-tum-eval-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 9.78 & 38.00 & 68.78 & 46.09 & 61.91 \\
0 & 0 & -- & A1 & 9.78 & 38.00 & 68.78 & 46.09 & 61.91 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 11.56 & 32.56 & 65.78 & 43.01 & 58.71 \\
30 & 0 & -- & A1 & 11.56 & 32.56 & 65.78 & 43.01 & 58.71 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 10.22 & 32.78 & 67.33 & 43.47 & 59.53 \\
50 & 0 & -- & A1 & 10.22 & 32.78 & 67.33 & 43.47 & 59.53 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 10.11 & 33.22 & 67.67 & 43.19 & 59.56 \\
70 & 0 & -- & A1 & 10.11 & 33.22 & 67.67 & 43.19 & 59.56 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 11.78 & 32.00 & 71.00 & 44.97 & 62.44 \\
100 & 0 & -- & A1 & 11.78 & 32.00 & 71.00 & 44.97 & 62.44 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 6.33 & 35.78 & 71.00 & 46.42 & 61.81 \\
0 & 30 & GT & A1 & \textbf{6.67} & \textbf{36.56} & \textbf{72.00} & \textbf{47.17} & \textbf{62.24} \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 7.00 & 36.89 & 74.00 & 48.24 & 63.81 \\
0 & 50 & GT & A1 & \textbf{9.11} & \textbf{39.00} & \textbf{74.67} & \textbf{49.33} & \textbf{64.37} \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 16.78 & 47.22 & 77.22 & 54.07 & 68.23 \\
0 & 70 & GT & A1 & \textbf{19.89} & \textbf{49.67} & \textbf{78.33} & \textbf{56.62} & \textbf{69.60} \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 45.56 & 70.78 & 82.44 & 70.36 & 78.90 \\
0 & 100 & GT & A1 & \textbf{46.00} & \textbf{72.22} & \textbf{86.56} & \textbf{72.98} & \textbf{80.99} \\
\addlinespace[1pt]
0 & 30 & N & A0 & \textbf{6.22} & 34.00 & 70.22 & 45.20 & 60.94 \\
0 & 30 & N & A1 & 6.11 & \textbf{35.11} & \textbf{71.11} & \textbf{45.97} & \textbf{61.46} \\
\addlinespace[1pt]
0 & 50 & N & A0 & 3.78 & 33.89 & 72.67 & 46.43 & 62.27 \\
0 & 50 & N & A1 & \textbf{5.11} & \textbf{34.44} & \textbf{73.67} & \textbf{46.84} & \textbf{62.53} \\
\addlinespace[1pt]
0 & 70 & N & A0 & \textbf{10.00} & 40.89 & 73.78 & 50.23 & 65.19 \\
0 & 70 & N & A1 & 9.67 & \textbf{41.44} & \textbf{74.56} & \textbf{50.47} & \textbf{65.82} \\
\addlinespace[1pt]
0 & 100 & N & A0 & \textbf{25.56} & \textbf{58.89} & 79.11 & \textbf{61.99} & 72.20 \\
0 & 100 & N & A1 & 22.11 & 56.44 & \textbf{80.00} & 61.34 & \textbf{73.40} \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 38.89 & 67.67 & 81.00 & 67.33 & 76.40 \\
100 & 100 & GT & A1 & \textbf{42.44} & \textbf{71.89} & \textbf{82.11} & \textbf{69.74} & \textbf{77.74} \\
\addlinespace[1pt]
100 & 100 & N & A0 & \textbf{24.22} & 57.11 & \textbf{79.00} & \textbf{60.65} & 71.30 \\
100 & 100 & N & A1 & 23.22 & \textbf{57.56} & 78.22 & 60.47 & \textbf{71.32} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_tum-eval_pose.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, released-weight intervention. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:released-tum-eval-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 96.11 & 99.67 & 100.00 & 9.78 & 38.00 & 68.78 & 46.09 & 61.94 \\
0 & 0 & -- & A1 & 96.11 & 99.67 & 100.00 & 9.78 & 38.00 & 68.78 & 46.09 & 61.94 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 96.78 & 97.22 & 100.00 & 11.56 & 32.56 & 65.78 & 43.01 & 58.76 \\
30 & 0 & -- & A1 & 96.78 & 97.22 & 100.00 & 11.56 & 32.56 & 65.78 & 43.01 & 58.76 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 96.67 & 97.22 & 97.78 & 10.22 & 32.78 & 67.56 & 43.52 & 59.70 \\
50 & 0 & -- & A1 & 96.67 & 97.22 & 97.78 & 10.22 & 32.78 & 67.56 & 43.52 & 59.70 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 96.44 & 97.11 & 99.89 & 10.11 & 33.22 & 67.78 & 43.21 & 59.64 \\
70 & 0 & -- & A1 & 96.44 & 97.11 & 99.89 & 10.11 & 33.22 & 67.78 & 43.21 & 59.64 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 96.78 & 96.89 & 97.22 & 11.78 & 32.00 & 71.11 & 44.97 & 62.54 \\
100 & 0 & -- & A1 & 96.78 & 96.89 & 97.22 & 11.78 & 32.00 & 71.11 & 44.97 & 62.54 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & \textbf{96.44} & 97.78 & 100.00 & 6.33 & 35.78 & 71.00 & 46.42 & 62.17 \\
0 & 30 & GT & A1 & 96.33 & 97.78 & 100.00 & \textbf{6.67} & \textbf{36.56} & \textbf{72.22} & \textbf{47.22} & \textbf{62.53} \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 96.78 & 97.78 & 100.00 & 7.00 & 36.89 & 74.00 & 48.24 & 63.90 \\
0 & 50 & GT & A1 & 96.78 & 97.78 & 100.00 & \textbf{9.11} & \textbf{39.00} & \textbf{74.67} & \textbf{49.33} & \textbf{64.50} \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 97.67 & \textbf{97.78} & 100.00 & 16.78 & 47.22 & 77.22 & 54.07 & 68.32 \\
0 & 70 & GT & A1 & 97.67 & 97.67 & 100.00 & \textbf{19.89} & \textbf{49.67} & \textbf{78.44} & \textbf{56.63} & \textbf{69.86} \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 97.00 & 100.00 & 100.00 & 45.56 & 70.78 & 82.44 & 70.36 & 78.95 \\
0 & 100 & GT & A1 & \textbf{99.44} & 100.00 & 100.00 & \textbf{46.00} & \textbf{72.22} & \textbf{86.56} & \textbf{72.98} & \textbf{81.03} \\
\addlinespace[1pt]
0 & 30 & N & A0 & \textbf{96.44} & 97.78 & 100.00 & \textbf{6.22} & 34.00 & 70.22 & 45.20 & 61.19 \\
0 & 30 & N & A1 & 96.33 & 97.78 & 100.00 & 6.11 & \textbf{35.11} & \textbf{71.22} & \textbf{45.98} & \textbf{61.65} \\
\addlinespace[1pt]
0 & 50 & N & A0 & 96.78 & 97.78 & 100.00 & 3.78 & 33.89 & 72.78 & 46.48 & 62.47 \\
0 & 50 & N & A1 & 96.78 & 97.78 & 100.00 & \textbf{5.11} & \textbf{34.44} & \textbf{73.67} & \textbf{46.84} & \textbf{62.66} \\
\addlinespace[1pt]
0 & 70 & N & A0 & 97.67 & \textbf{98.00} & 100.00 & \textbf{10.00} & 40.89 & 74.22 & 50.36 & 65.53 \\
0 & 70 & N & A1 & 97.67 & 97.67 & 100.00 & 9.67 & \textbf{41.67} & \textbf{75.00} & \textbf{50.71} & \textbf{66.34} \\
\addlinespace[1pt]
0 & 100 & N & A0 & 97.22 & 100.00 & 100.00 & \textbf{25.56} & \textbf{58.89} & 79.11 & \textbf{61.99} & 72.21 \\
0 & 100 & N & A1 & \textbf{100.00} & 100.00 & 100.00 & 22.11 & 56.44 & \textbf{80.00} & 61.34 & \textbf{73.50} \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 96.89 & 97.22 & 100.00 & 39.00 & 67.78 & 81.22 & 67.50 & 76.66 \\
100 & 100 & GT & A1 & \textbf{97.11} & \textbf{100.00} & 100.00 & \textbf{42.44} & \textbf{71.89} & \textbf{82.22} & \textbf{69.75} & \textbf{77.81} \\
\addlinespace[1pt]
100 & 100 & N & A0 & 96.89 & 97.22 & 100.00 & \textbf{24.22} & 57.11 & \textbf{79.00} & \textbf{60.65} & 71.30 \\
100 & 100 & N & A1 & \textbf{97.22} & \textbf{100.00} & 100.00 & 23.22 & \textbf{57.56} & 78.22 & 60.47 & \textbf{71.32} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_tum-eval_retention.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:released-tum-eval-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 60 & 60 \\
0 & 30 & GT & A0 & 100.00 & 100.00 & 8.33 & 40.00 & 50.78 & 66.83 & 60 & 60 \\
0 & 30 & GT & A1 & 100.00 & 100.00 & 13.33 & 50.00 & 56.11 & 69.11 & 60 & 60 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 200 & 200 \\
0 & 50 & GT & A0 & 100.00 & 100.00 & 18.50 & 55.00 & 58.93 & 72.60 & 200 & 200 \\
0 & 50 & GT & A1 & 100.00 & 100.00 & 26.00 & 59.50 & 63.10 & 75.33 & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 420 & 420 \\
0 & 70 & GT & A0 & 100.00 & 100.00 & 32.86 & 66.43 & 66.51 & 77.75 & 420 & 420 \\
0 & 70 & GT & A1 & 100.00 & 100.00 & 38.10 & 70.24 & 71.54 & 81.17 & 420 & 420 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 900 & 900 \\
0 & 100 & GT & A0 & 97.00 & 100.00 & 45.56 & 70.78 & 70.36 & 78.95 & 900 & 900 \\
0 & 100 & GT & A1 & 99.44 & 100.00 & 46.00 & 72.22 & 72.98 & 81.03 & 900 & 900 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 21.67 & 63.33 & 65.78 & 80.56 & 60 & 60 \\
0 & 30 & N & A0 & 100.00 & 100.00 & 5.00 & 21.67 & 43.56 & 61.78 & 60 & 60 \\
0 & 30 & N & A1 & 100.00 & 100.00 & 5.00 & 31.67 & 47.00 & 63.50 & 60 & 60 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 24.00 & 64.50 & 68.97 & 83.52 & 200 & 200 \\
0 & 50 & N & A0 & 100.00 & 100.00 & 5.00 & 40.50 & 53.30 & 68.65 & 200 & 200 \\
0 & 50 & N & A1 & 100.00 & 100.00 & 9.00 & 44.00 & 54.83 & 69.55 & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 26.19 & 65.71 & 68.27 & 82.75 & 420 & 420 \\
0 & 70 & N & A0 & 100.00 & 100.00 & 17.62 & 54.05 & 59.48 & 72.54 & 420 & 420 \\
0 & 70 & N & A1 & 100.00 & 100.00 & 15.95 & 54.29 & 59.92 & 74.37 & 420 & 420 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 100.00 & 100.00 & 26.44 & 66.00 & 67.87 & 81.07 & 900 & 900 \\
0 & 100 & N & A0 & 97.22 & 100.00 & 25.56 & 58.89 & 61.99 & 72.21 & 900 & 900 \\
0 & 100 & N & A1 & 100.00 & 100.00 & 22.11 & 56.44 & 61.34 & 73.50 & 900 & 900 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 900 & 900 \\
100 & 100 & GT & A0 & 96.89 & 97.22 & 39.00 & 67.78 & 67.50 & 76.66 & 900 & 900 \\
100 & 100 & GT & A1 & 97.11 & 100.00 & 42.44 & 71.89 & 69.75 & 77.81 & 900 & 900 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 100.00 & 100.00 & 26.44 & 66.00 & 67.87 & 81.07 & 900 & 900 \\
100 & 100 & N & A0 & 96.89 & 97.22 & 24.22 & 57.11 & 60.65 & 71.30 & 900 & 900 \\
100 & 100 & N & A1 & 97.22 & 100.00 & 23.22 & 57.56 & 60.47 & 71.32 & 900 & 900 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_v2_depth.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, released-weight intervention. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:released-v2-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & A0 & 0.106 & 89.88 & 0.106 & 89.88 & 2.50e-01 & 6600 & 6600 \\
0 & 0 & -- & A1 & 0.106 & 89.88 & 0.106 & 89.88 & 2.50e-01 & 6600 & 6600 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 0.072 & 93.47 & 0.088 & 91.41 & 2.65e-01 & 6600 & 4620 \\
30 & 0 & -- & A1 & 0.072 & 93.47 & 0.088 & 91.41 & 2.65e-01 & 6600 & 4620 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 0.059 & 95.03 & 0.085 & 91.71 & 2.62e-01 & 6600 & 3300 \\
50 & 0 & -- & A1 & 0.059 & 95.03 & 0.085 & 91.71 & 2.62e-01 & 6600 & 3300 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 0.046 & 96.62 & 0.079 & 92.52 & 2.71e-01 & 6600 & 1980 \\
70 & 0 & -- & A1 & 0.046 & 96.62 & 0.079 & 92.52 & 2.71e-01 & 6600 & 1980 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 0.031 & 98.43 & -- & -- & 2.74e-01 & 6600 & 0 \\
100 & 0 & -- & A1 & 0.031 & 98.43 & -- & -- & 2.74e-01 & 6600 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 0.105 & 89.90 & 0.105 & 89.90 & 2.72e-01 & 6600 & 6600 \\
0 & 30 & GT & A1 & 0.105 & 89.90 & 0.105 & 89.90 & \textbf{2.70e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 0.105 & 89.96 & 0.105 & 89.96 & 2.61e-01 & 6600 & 6600 \\
0 & 50 & GT & A1 & 0.105 & 89.96 & 0.105 & 89.96 & \textbf{2.57e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 0.104 & 90.01 & 0.104 & 90.01 & 2.36e-01 & 6600 & 6600 \\
0 & 70 & GT & A1 & 0.104 & 90.01 & 0.104 & 90.01 & \textbf{2.30e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 0.104 & 90.05 & 0.104 & 90.05 & 6.35e-02 & 6600 & 6600 \\
0 & 100 & GT & A1 & 0.104 & 90.05 & 0.104 & 90.05 & \textbf{4.38e-02} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 30 & N & A0 & 0.105 & 89.90 & 0.105 & 89.90 & 2.73e-01 & 6600 & 6600 \\
0 & 30 & N & A1 & 0.105 & 89.90 & 0.105 & 89.90 & \textbf{2.71e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 50 & N & A0 & 0.105 & 89.96 & 0.105 & 89.96 & 2.65e-01 & 6600 & 6600 \\
0 & 50 & N & A1 & 0.105 & 89.96 & 0.105 & 89.96 & \textbf{2.62e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & N & A0 & 0.104 & 90.01 & 0.104 & 90.01 & 2.44e-01 & 6600 & 6600 \\
0 & 70 & N & A1 & 0.104 & 90.01 & 0.104 & 90.01 & \textbf{2.41e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 100 & N & A0 & 0.104 & 90.05 & 0.104 & 90.05 & 7.03e-02 & 6600 & 6600 \\
0 & 100 & N & A1 & 0.104 & 90.05 & 0.104 & 90.05 & \textbf{5.40e-02} & 6600 & 6600 \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 0.031 & 98.43 & -- & -- & 6.04e-02 & 6600 & 0 \\
100 & 100 & GT & A1 & 0.031 & 98.43 & -- & -- & \textbf{4.56e-02} & 6600 & 0 \\
\addlinespace[1pt]
100 & 100 & N & A0 & 0.031 & 98.43 & -- & -- & 6.72e-02 & 6600 & 0 \\
100 & 100 & N & A1 & 0.031 & 98.43 & -- & -- & \textbf{5.49e-02} & 6600 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_v2_directed.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, released-weight intervention. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:released-v2-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 15.77 & 55.59 & 89.60 & 62.33 & 77.57 \\
0 & 0 & -- & A1 & 15.77 & 55.59 & 89.60 & 62.33 & 77.57 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 13.30 & 51.20 & 88.63 & 60.15 & 76.23 \\
30 & 0 & -- & A1 & 13.30 & 51.20 & 88.63 & 60.15 & 76.23 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 12.80 & 50.14 & 88.29 & 59.58 & 75.88 \\
50 & 0 & -- & A1 & 12.80 & 50.14 & 88.29 & 59.58 & 75.88 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 12.98 & 49.94 & 88.08 & 59.52 & 75.66 \\
70 & 0 & -- & A1 & 12.98 & 49.94 & 88.08 & 59.52 & 75.66 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 12.55 & 49.96 & 88.34 & 59.91 & 75.87 \\
100 & 0 & -- & A1 & 12.55 & 49.96 & 88.34 & 59.91 & 75.87 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 20.35 & 58.76 & 89.38 & 63.55 & 78.05 \\
0 & 30 & GT & A1 & \textbf{20.76} & \textbf{59.46} & \textbf{89.62} & \textbf{64.05} & \textbf{78.36} \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 28.70 & 64.24 & 90.55 & 67.12 & 80.31 \\
0 & 50 & GT & A1 & \textbf{29.71} & \textbf{64.86} & \textbf{91.04} & \textbf{67.97} & \textbf{80.85} \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 42.37 & 73.18 & 92.16 & 73.28 & 83.96 \\
0 & 70 & GT & A1 & \textbf{45.00} & \textbf{73.79} & \textbf{92.55} & \textbf{74.62} & \textbf{84.77} \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 69.55 & 92.63 & 98.50 & 88.74 & 93.88 \\
0 & 100 & GT & A1 & \textbf{79.36} & \textbf{94.94} & \textbf{99.26} & \textbf{92.57} & \textbf{96.09} \\
\addlinespace[1pt]
0 & 30 & N & A0 & \textbf{19.07} & 58.01 & 89.16 & 62.99 & 77.73 \\
0 & 30 & N & A1 & 19.01 & \textbf{58.20} & \textbf{89.18} & \textbf{63.15} & \textbf{77.82} \\
\addlinespace[1pt]
0 & 50 & N & A0 & \textbf{23.21} & \textbf{61.07} & 89.95 & \textbf{64.80} & \textbf{79.02} \\
0 & 50 & N & A1 & 22.29 & 60.44 & \textbf{90.01} & 64.63 & 78.98 \\
\addlinespace[1pt]
0 & 70 & N & A0 & \textbf{29.10} & \textbf{66.71} & \textbf{90.99} & \textbf{68.35} & \textbf{81.23} \\
0 & 70 & N & A1 & 27.29 & 65.54 & 90.83 & 67.84 & 80.99 \\
\addlinespace[1pt]
0 & 100 & N & A0 & \textbf{40.06} & \textbf{80.41} & 97.05 & 79.45 & 88.94 \\
0 & 100 & N & A1 & 39.13 & 80.40 & \textbf{97.46} & \textbf{79.85} & \textbf{89.37} \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 69.15 & 91.68 & 98.28 & 88.26 & 93.65 \\
100 & 100 & GT & A1 & \textbf{77.06} & \textbf{93.85} & \textbf{99.18} & \textbf{91.79} & \textbf{95.70} \\
\addlinespace[1pt]
100 & 100 & N & A0 & 38.90 & 80.04 & 96.96 & 79.08 & 88.76 \\
100 & 100 & N & A1 & \textbf{39.69} & \textbf{80.20} & \textbf{97.42} & \textbf{79.90} & \textbf{89.40} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_v2_pose.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, released-weight intervention. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:released-v2-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 61.49 & 89.96 & 96.92 & 15.77 & 55.60 & 89.78 & 62.37 & 77.68 \\
0 & 0 & -- & A1 & 61.49 & 89.96 & 96.92 & 15.77 & 55.60 & 89.78 & 62.37 & 77.68 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 63.79 & 90.31 & 97.10 & 13.32 & 51.25 & 88.95 & 60.26 & 76.47 \\
30 & 0 & -- & A1 & 63.79 & 90.31 & 97.10 & 13.32 & 51.25 & 88.95 & 60.26 & 76.47 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 64.98 & 90.49 & 96.94 & 12.81 & 50.20 & 88.63 & 59.69 & 76.14 \\
50 & 0 & -- & A1 & 64.98 & 90.49 & 96.94 & 12.81 & 50.20 & 88.63 & 59.69 & 76.14 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 66.09 & 90.31 & 96.70 & 12.99 & 50.00 & 88.42 & 59.63 & 75.93 \\
70 & 0 & -- & A1 & 66.09 & 90.31 & 96.70 & 12.99 & 50.00 & 88.42 & 59.63 & 75.93 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 68.11 & 90.87 & 96.69 & 12.56 & 50.01 & 88.64 & 60.01 & 76.09 \\
100 & 0 & -- & A1 & 68.11 & 90.87 & 96.69 & 12.56 & 50.01 & 88.64 & 60.01 & 76.09 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 61.98 & 90.12 & 96.83 & 20.35 & 58.79 & 89.61 & 63.60 & 78.21 \\
0 & 30 & GT & A1 & \textbf{62.96} & \textbf{90.18} & \textbf{96.85} & \textbf{20.76} & \textbf{59.49} & \textbf{89.85} & \textbf{64.11} & \textbf{78.51} \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 63.11 & 90.37 & 97.09 & 28.70 & 64.26 & 90.75 & 67.18 & 80.46 \\
0 & 50 & GT & A1 & \textbf{64.46} & \textbf{90.43} & \textbf{97.19} & \textbf{29.73} & \textbf{64.89} & \textbf{91.25} & \textbf{68.03} & \textbf{81.00} \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 70.02 & 91.78 & 97.55 & 42.38 & 73.19 & 92.29 & 73.32 & 84.08 \\
0 & 70 & GT & A1 & \textbf{71.82} & \textbf{92.07} & \textbf{97.75} & \textbf{45.01} & \textbf{73.81} & \textbf{92.66} & \textbf{74.66} & \textbf{84.88} \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 93.39 & 97.75 & 99.36 & 69.55 & 92.63 & 98.51 & 88.74 & 93.88 \\
0 & 100 & GT & A1 & \textbf{98.32} & \textbf{99.57} & \textbf{100.00} & \textbf{79.36} & \textbf{94.94} & \textbf{99.26} & \textbf{92.57} & \textbf{96.09} \\
\addlinespace[1pt]
0 & 30 & N & A0 & 61.99 & 90.10 & 96.81 & \textbf{19.07} & 58.04 & 89.39 & 63.05 & 77.88 \\
0 & 30 & N & A1 & \textbf{62.90} & \textbf{90.13} & \textbf{96.84} & 19.02 & \textbf{58.24} & \textbf{89.42} & \textbf{63.21} & \textbf{77.98} \\
\addlinespace[1pt]
0 & 50 & N & A0 & 63.02 & 90.31 & 97.10 & \textbf{23.22} & \textbf{61.09} & 90.14 & \textbf{64.85} & \textbf{79.16} \\
0 & 50 & N & A1 & \textbf{64.17} & \textbf{90.39} & \textbf{97.19} & 22.30 & 60.46 & \textbf{90.19} & 64.68 & 79.12 \\
\addlinespace[1pt]
0 & 70 & N & A0 & 69.81 & 91.72 & 97.55 & \textbf{29.10} & \textbf{66.73} & \textbf{91.10} & \textbf{68.38} & \textbf{81.35} \\
0 & 70 & N & A1 & \textbf{71.43} & \textbf{91.98} & \textbf{97.75} & 27.30 & 65.56 & 90.92 & 67.87 & 81.09 \\
\addlinespace[1pt]
0 & 100 & N & A0 & 93.10 & 97.74 & 99.35 & \textbf{40.06} & \textbf{80.41} & 97.05 & 79.45 & 88.94 \\
0 & 100 & N & A1 & \textbf{97.90} & \textbf{99.58} & \textbf{100.00} & 39.13 & 80.40 & \textbf{97.46} & \textbf{79.85} & \textbf{89.37} \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 93.83 & 97.28 & 99.24 & 69.15 & 91.68 & 98.28 & 88.26 & 93.65 \\
100 & 100 & GT & A1 & \textbf{97.85} & \textbf{99.45} & \textbf{100.00} & \textbf{77.06} & \textbf{93.85} & \textbf{99.18} & \textbf{91.79} & \textbf{95.70} \\
\addlinespace[1pt]
100 & 100 & N & A0 & 93.51 & 97.22 & 99.24 & 38.90 & 80.04 & 96.96 & 79.08 & 88.76 \\
100 & 100 & N & A1 & \textbf{97.54} & \textbf{99.46} & \textbf{100.00} & \textbf{39.69} & \textbf{80.20} & \textbf{97.42} & \textbf{79.90} & \textbf{89.40} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_v2_retention.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:released-v2-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 1980 & 1980 \\
0 & 30 & GT & A0 & 98.48 & 99.34 & 54.09 & 84.19 & 82.65 & 90.40 & 1980 & 1980 \\
0 & 30 & GT & A1 & 99.44 & 99.80 & 55.10 & 85.61 & 84.99 & 92.20 & 1980 & 1980 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 6600 & 6600 \\
0 & 50 & GT & A0 & 97.42 & 98.98 & 63.74 & 90.47 & 87.26 & 93.14 & 6600 & 6600 \\
0 & 50 & GT & A1 & 98.88 & 99.52 & 67.67 & 91.94 & 89.73 & 94.68 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 13860 & 13860 \\
0 & 70 & GT & A0 & 96.35 & 98.75 & 68.14 & 92.81 & 88.94 & 94.14 & 13860 & 13860 \\
0 & 70 & GT & A1 & 98.87 & 99.56 & 74.02 & 94.11 & 91.50 & 95.56 & 13860 & 13860 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 29700 & 29700 \\
0 & 100 & GT & A0 & 93.39 & 97.75 & 69.55 & 92.63 & 88.74 & 93.88 & 29700 & 29700 \\
0 & 100 & GT & A1 & 98.32 & 99.57 & 79.36 & 94.94 & 92.57 & 96.09 & 29700 & 29700 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 49.39 & 82.93 & 82.16 & 90.67 & 1980 & 1980 \\
0 & 30 & N & A0 & 98.48 & 99.34 & 38.84 & 74.65 & 75.86 & 86.64 & 1980 & 1980 \\
0 & 30 & N & A1 & 99.44 & 99.80 & 34.24 & 73.43 & 75.37 & 86.88 & 1980 & 1980 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 48.68 & 83.64 & 82.60 & 90.97 & 6600 & 6600 \\
0 & 50 & N & A0 & 97.29 & 98.98 & 41.11 & 79.23 & 78.92 & 88.73 & 6600 & 6600 \\
0 & 50 & N & A1 & 98.83 & 99.52 & 38.29 & 77.26 & 78.18 & 88.53 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 47.98 & 83.95 & 82.69 & 91.00 & 13860 & 13860 \\
0 & 70 & N & A0 & 96.20 & 98.73 & 40.84 & 80.66 & 79.77 & 89.28 & 13860 & 13860 \\
0 & 70 & N & A1 & 98.72 & 99.56 & 37.99 & 78.95 & 78.99 & 88.92 & 13860 & 13860 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 99.85 & 100.00 & 47.41 & 84.00 & 82.72 & 91.01 & 29700 & 29700 \\
0 & 100 & N & A0 & 93.10 & 97.74 & 40.06 & 80.41 & 79.45 & 88.94 & 29700 & 29700 \\
0 & 100 & N & A1 & 97.90 & 99.58 & 39.13 & 80.40 & 79.85 & 89.37 & 29700 & 29700 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 29700 & 29700 \\
100 & 100 & GT & A0 & 93.83 & 97.28 & 69.15 & 91.68 & 88.26 & 93.65 & 29700 & 29700 \\
100 & 100 & GT & A1 & 97.85 & 99.45 & 77.06 & 93.85 & 91.79 & 95.70 & 29700 & 29700 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 99.85 & 100.00 & 47.41 & 84.00 & 82.72 & 91.01 & 29700 & 29700 \\
100 & 100 & N & A0 & 93.51 & 97.22 & 38.90 & 80.04 & 79.08 & 88.76 & 29700 & 29700 \\
100 & 100 & N & A1 & 97.54 & 99.46 & 39.69 & 80.20 & 79.90 & 89.40 & 29700 & 29700 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_vkitti-eval_depth.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, released-weight intervention. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:released-vkitti-eval-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & A0 & 0.078 & 92.65 & 0.078 & 92.65 & 5.45e-02 & 700 & 700 \\
0 & 0 & -- & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 5.45e-02 & 700 & 700 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 0.077 & 92.95 & 0.077 & 92.77 & 6.68e-02 & 700 & 490 \\
30 & 0 & -- & A1 & 0.077 & 92.95 & 0.077 & 92.77 & 6.68e-02 & 700 & 490 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 0.076 & 93.18 & 0.076 & 92.83 & 6.79e-02 & 700 & 350 \\
50 & 0 & -- & A1 & 0.076 & 93.18 & 0.076 & 92.83 & 6.79e-02 & 700 & 350 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 0.075 & 93.40 & 0.075 & 92.87 & 7.60e-02 & 700 & 210 \\
70 & 0 & -- & A1 & 0.075 & 93.40 & 0.075 & 92.87 & 7.60e-02 & 700 & 210 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 0.074 & 93.75 & -- & -- & 2.32e-01 & 700 & 0 \\
100 & 0 & -- & A1 & 0.074 & 93.75 & -- & -- & 2.32e-01 & 700 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{8.26e-02} & 700 & 700 \\
0 & 30 & GT & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 1.09e-01 & 700 & 700 \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{8.72e-02} & 700 & 700 \\
0 & 50 & GT & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 9.92e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{9.43e-02} & 700 & 700 \\
0 & 70 & GT & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 1.00e-01 & 700 & 700 \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 0.078 & 92.65 & 0.078 & 92.65 & 3.24e-02 & 700 & 700 \\
0 & 100 & GT & A1 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{3.09e-02} & 700 & 700 \\
\addlinespace[1pt]
0 & 30 & N & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{8.29e-02} & 700 & 700 \\
0 & 30 & N & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 1.09e-01 & 700 & 700 \\
\addlinespace[1pt]
0 & 50 & N & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{8.80e-02} & 700 & 700 \\
0 & 50 & N & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 1.00e-01 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & N & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{9.57e-02} & 700 & 700 \\
0 & 70 & N & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 1.01e-01 & 700 & 700 \\
\addlinespace[1pt]
0 & 100 & N & A0 & 0.078 & 92.65 & 0.078 & 92.65 & \textbf{3.50e-02} & 700 & 700 \\
0 & 100 & N & A1 & 0.078 & 92.65 & 0.078 & 92.65 & 3.58e-02 & 700 & 700 \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 0.074 & 93.75 & -- & -- & 2.89e-02 & 700 & 0 \\
100 & 100 & GT & A1 & 0.074 & 93.75 & -- & -- & \textbf{2.70e-02} & 700 & 0 \\
\addlinespace[1pt]
100 & 100 & N & A0 & 0.074 & 93.75 & -- & -- & \textbf{3.19e-02} & 700 & 0 \\
100 & 100 & N & A1 & 0.074 & 93.75 & -- & -- & 3.28e-02 & 700 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_vkitti-eval_directed.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, released-weight intervention. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:released-vkitti-eval-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 97.21 & 99.52 & 99.81 & 97.86 & 98.86 \\
0 & 0 & -- & A1 & 97.21 & 99.52 & 99.81 & 97.86 & 98.86 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 94.00 & 99.43 & 99.78 & 97.09 & 98.48 \\
30 & 0 & -- & A1 & 94.00 & 99.43 & 99.78 & 97.09 & 98.48 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 92.63 & 99.24 & 99.78 & 96.85 & 98.36 \\
50 & 0 & -- & A1 & 92.63 & 99.24 & 99.78 & 96.85 & 98.36 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 93.87 & 98.92 & 99.84 & 96.80 & 98.33 \\
70 & 0 & -- & A1 & 93.87 & 98.92 & 99.84 & 96.80 & 98.33 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 94.79 & 98.57 & 99.27 & 97.03 & 98.19 \\
100 & 0 & -- & A1 & 94.79 & 98.57 & 99.27 & 97.03 & 98.19 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & \textbf{97.24} & \textbf{99.46} & \textbf{99.84} & \textbf{98.19} & \textbf{99.03} \\
0 & 30 & GT & A1 & 96.22 & 99.43 & 99.81 & 98.02 & 98.94 \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 95.30 & 99.30 & \textbf{99.84} & 97.75 & 98.82 \\
0 & 50 & GT & A1 & \textbf{95.94} & \textbf{99.33} & 99.81 & \textbf{98.06} & \textbf{98.96} \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 91.71 & 98.29 & \textbf{99.84} & 97.21 & 98.55 \\
0 & 70 & GT & A1 & \textbf{93.84} & \textbf{98.95} & 99.81 & \textbf{97.81} & \textbf{98.85} \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 99.59 & 99.81 & 99.84 & 99.56 & 99.74 \\
0 & 100 & GT & A1 & \textbf{99.75} & 99.81 & \textbf{99.90} & \textbf{99.71} & \textbf{99.84} \\
\addlinespace[1pt]
0 & 30 & N & A0 & \textbf{97.05} & \textbf{99.46} & \textbf{99.84} & \textbf{98.14} & \textbf{99.00} \\
0 & 30 & N & A1 & 95.97 & 99.40 & 99.81 & 97.97 & 98.91 \\
\addlinespace[1pt]
0 & 50 & N & A0 & 95.27 & 99.30 & \textbf{99.84} & 97.67 & 98.78 \\
0 & 50 & N & A1 & \textbf{95.87} & \textbf{99.33} & 99.81 & \textbf{97.96} & \textbf{98.91} \\
\addlinespace[1pt]
0 & 70 & N & A0 & 91.81 & 98.32 & \textbf{99.84} & 97.03 & 98.46 \\
0 & 70 & N & A1 & \textbf{93.87} & \textbf{98.83} & 99.81 & \textbf{97.67} & \textbf{98.78} \\
\addlinespace[1pt]
0 & 100 & N & A0 & 99.52 & 99.78 & 99.87 & 99.36 & 99.64 \\
0 & 100 & N & A1 & \textbf{99.78} & \textbf{99.81} & \textbf{99.90} & \textbf{99.51} & \textbf{99.73} \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 99.59 & \textbf{99.81} & 99.87 & 99.04 & 99.50 \\
100 & 100 & GT & A1 & \textbf{99.78} & 99.78 & \textbf{99.94} & \textbf{99.54} & \textbf{99.75} \\
\addlinespace[1pt]
100 & 100 & N & A0 & 99.24 & 99.78 & 99.87 & 98.44 & 99.18 \\
100 & 100 & N & A1 & \textbf{99.68} & 99.78 & 99.87 & \textbf{99.15} & \textbf{99.55} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_vkitti-eval_pose.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, released-weight intervention. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:released-vkitti-eval-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & A0 & 100.00 & 100.00 & 100.00 & 97.21 & 99.52 & 99.81 & 97.86 & 98.86 \\
0 & 0 & -- & A1 & 100.00 & 100.00 & 100.00 & 97.21 & 99.52 & 99.81 & 97.86 & 98.86 \\
\addlinespace[1pt]
30 & 0 & -- & A0 & 100.00 & 100.00 & 100.00 & 94.00 & 99.43 & 99.78 & 97.09 & 98.48 \\
30 & 0 & -- & A1 & 100.00 & 100.00 & 100.00 & 94.00 & 99.43 & 99.78 & 97.09 & 98.48 \\
\addlinespace[1pt]
50 & 0 & -- & A0 & 100.00 & 100.00 & 100.00 & 92.63 & 99.24 & 99.78 & 96.85 & 98.36 \\
50 & 0 & -- & A1 & 100.00 & 100.00 & 100.00 & 92.63 & 99.24 & 99.78 & 96.85 & 98.36 \\
\addlinespace[1pt]
70 & 0 & -- & A0 & 100.00 & 100.00 & 100.00 & 93.87 & 98.92 & 99.84 & 96.80 & 98.33 \\
70 & 0 & -- & A1 & 100.00 & 100.00 & 100.00 & 93.87 & 98.92 & 99.84 & 96.80 & 98.33 \\
\addlinespace[1pt]
100 & 0 & -- & A0 & 99.14 & 100.00 & 100.00 & 94.79 & 98.63 & 99.49 & 97.17 & 98.39 \\
100 & 0 & -- & A1 & 99.14 & 100.00 & 100.00 & 94.79 & 98.63 & 99.49 & 97.17 & 98.39 \\
\addlinespace[1pt]
0 & 30 & GT & A0 & 100.00 & 100.00 & 100.00 & \textbf{97.24} & \textbf{99.46} & \textbf{99.84} & \textbf{98.19} & \textbf{99.03} \\
0 & 30 & GT & A1 & 100.00 & 100.00 & 100.00 & 96.22 & 99.43 & 99.81 & 98.02 & 98.94 \\
\addlinespace[1pt]
0 & 50 & GT & A0 & 100.00 & 100.00 & 100.00 & 95.30 & 99.30 & \textbf{99.84} & 97.75 & 98.82 \\
0 & 50 & GT & A1 & 100.00 & 100.00 & 100.00 & \textbf{95.94} & \textbf{99.33} & 99.81 & \textbf{98.06} & \textbf{98.96} \\
\addlinespace[1pt]
0 & 70 & GT & A0 & 100.00 & 100.00 & 100.00 & 91.71 & 98.29 & \textbf{99.84} & 97.21 & 98.55 \\
0 & 70 & GT & A1 & 100.00 & 100.00 & 100.00 & \textbf{93.84} & \textbf{98.95} & 99.81 & \textbf{97.81} & \textbf{98.85} \\
\addlinespace[1pt]
0 & 100 & GT & A0 & 100.00 & 100.00 & 100.00 & 99.59 & 99.81 & 99.84 & 99.56 & 99.74 \\
0 & 100 & GT & A1 & 100.00 & 100.00 & 100.00 & \textbf{99.75} & 99.81 & \textbf{99.90} & \textbf{99.71} & \textbf{99.84} \\
\addlinespace[1pt]
0 & 30 & N & A0 & 100.00 & 100.00 & 100.00 & \textbf{97.05} & \textbf{99.46} & \textbf{99.84} & \textbf{98.14} & \textbf{99.00} \\
0 & 30 & N & A1 & 100.00 & 100.00 & 100.00 & 95.97 & 99.40 & 99.81 & 97.97 & 98.91 \\
\addlinespace[1pt]
0 & 50 & N & A0 & 100.00 & 100.00 & 100.00 & 95.27 & 99.30 & \textbf{99.84} & 97.67 & 98.78 \\
0 & 50 & N & A1 & 100.00 & 100.00 & 100.00 & \textbf{95.87} & \textbf{99.33} & 99.81 & \textbf{97.96} & \textbf{98.91} \\
\addlinespace[1pt]
0 & 70 & N & A0 & 100.00 & 100.00 & 100.00 & 91.81 & 98.32 & \textbf{99.84} & 97.03 & 98.46 \\
0 & 70 & N & A1 & 100.00 & 100.00 & 100.00 & \textbf{93.87} & \textbf{98.83} & 99.81 & \textbf{97.67} & \textbf{98.78} \\
\addlinespace[1pt]
0 & 100 & N & A0 & 100.00 & 100.00 & 100.00 & 99.52 & 99.78 & 99.87 & 99.36 & 99.64 \\
0 & 100 & N & A1 & 100.00 & 100.00 & 100.00 & \textbf{99.78} & \textbf{99.81} & \textbf{99.90} & \textbf{99.51} & \textbf{99.73} \\
\addlinespace[1pt]
100 & 100 & GT & A0 & 100.00 & 100.00 & 100.00 & 99.59 & \textbf{99.81} & 99.87 & 99.04 & 99.50 \\
100 & 100 & GT & A1 & 100.00 & 100.00 & 100.00 & \textbf{99.78} & 99.78 & \textbf{99.94} & \textbf{99.54} & \textbf{99.75} \\
\addlinespace[1pt]
100 & 100 & N & A0 & 100.00 & 100.00 & 100.00 & 99.24 & 99.78 & 99.87 & 98.44 & 99.18 \\
100 & 100 & N & A1 & 100.00 & 100.00 & 100.00 & \textbf{99.68} & 99.78 & 99.87 & \textbf{99.15} & \textbf{99.55} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/released_vkitti-eval_retention.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:released-vkitti-eval-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 210 & 210 \\
0 & 30 & GT & A0 & 100.00 & 100.00 & 99.05 & 100.00 & 99.11 & 99.56 & 210 & 210 \\
0 & 30 & GT & A1 & 100.00 & 100.00 & 85.24 & 100.00 & 95.78 & 97.89 & 210 & 210 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 700 & 700 \\
0 & 50 & GT & A0 & 100.00 & 100.00 & 100.00 & 100.00 & 99.60 & 99.80 & 700 & 700 \\
0 & 50 & GT & A1 & 100.00 & 100.00 & 99.71 & 100.00 & 99.48 & 99.74 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 1470 & 1470 \\
0 & 70 & GT & A0 & 100.00 & 100.00 & 100.00 & 100.00 & 99.76 & 99.88 & 1470 & 1470 \\
0 & 70 & GT & A1 & 100.00 & 100.00 & 100.00 & 100.00 & 99.85 & 99.92 & 1470 & 1470 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 3150 & 3150 \\
0 & 100 & GT & A0 & 100.00 & 100.00 & 99.59 & 99.81 & 99.56 & 99.74 & 3150 & 3150 \\
0 & 100 & GT & A1 & 100.00 & 100.00 & 99.75 & 99.81 & 99.71 & 99.84 & 3150 & 3150 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 99.84 & 99.92 & 210 & 210 \\
0 & 30 & N & A0 & 100.00 & 100.00 & 97.62 & 100.00 & 98.60 & 99.30 & 210 & 210 \\
0 & 30 & N & A1 & 100.00 & 100.00 & 85.24 & 100.00 & 95.49 & 97.75 & 210 & 210 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 99.93 & 99.97 & 700 & 700 \\
0 & 50 & N & A0 & 100.00 & 100.00 & 100.00 & 100.00 & 99.34 & 99.67 & 700 & 700 \\
0 & 50 & N & A1 & 100.00 & 100.00 & 99.29 & 100.00 & 98.99 & 99.50 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 99.95 & 99.98 & 1470 & 1470 \\
0 & 70 & N & A0 & 100.00 & 100.00 & 99.93 & 100.00 & 99.45 & 99.73 & 1470 & 1470 \\
0 & 70 & N & A1 & 100.00 & 100.00 & 100.00 & 100.00 & 99.52 & 99.76 & 1470 & 1470 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 100.00 & 100.00 & 99.78 & 99.90 & 99.89 & 99.95 & 3150 & 3150 \\
0 & 100 & N & A0 & 100.00 & 100.00 & 99.52 & 99.78 & 99.36 & 99.64 & 3150 & 3150 \\
0 & 100 & N & A1 & 100.00 & 100.00 & 99.78 & 99.81 & 99.51 & 99.73 & 3150 & 3150 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 3150 & 3150 \\
100 & 100 & GT & A0 & 100.00 & 100.00 & 99.59 & 99.81 & 99.04 & 99.50 & 3150 & 3150 \\
100 & 100 & GT & A1 & 100.00 & 100.00 & 99.78 & 99.78 & 99.54 & 99.75 & 3150 & 3150 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 100.00 & 100.00 & 99.78 & 99.90 & 99.89 & 99.95 & 3150 & 3150 \\
100 & 100 & N & A0 & 100.00 & 100.00 & 99.24 & 99.78 & 98.44 & 99.18 & 3150 & 3150 \\
100 & 100 & N & A1 & 100.00 & 100.00 & 99.68 & 99.78 & 99.15 & 99.55 & 3150 & 3150 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_c3vd-eval_depth.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, matched-training comparison. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-c3vd-eval-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & C1 & 0.055 & 97.87 & 0.055 & 97.87 & 7.89e-05 & 450 & 450 \\
0 & 0 & -- & C2 & 0.055 & \textbf{98.09} & 0.055 & \textbf{98.09} & \textbf{7.80e-05} & 450 & 450 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 0.015 & 99.78 & 0.020 & 99.70 & 9.27e-05 & 450 & 315 \\
30 & 0 & -- & C2 & 0.015 & \textbf{99.80} & \textbf{0.019} & \textbf{99.72} & \textbf{9.16e-05} & 450 & 315 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 0.011 & 99.86 & 0.017 & 99.75 & \textbf{9.48e-05} & 450 & 225 \\
50 & 0 & -- & C2 & \textbf{0.010} & \textbf{99.87} & 0.017 & 99.75 & 9.68e-05 & 450 & 225 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 0.007 & 99.92 & 0.015 & 99.77 & \textbf{1.02e-04} & 450 & 135 \\
70 & 0 & -- & C2 & 0.007 & 99.92 & \textbf{0.014} & \textbf{99.78} & 1.07e-04 & 450 & 135 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 0.004 & 99.98 & -- & -- & \textbf{4.13e-05} & 450 & 0 \\
100 & 0 & -- & C2 & 0.004 & 99.98 & -- & -- & 4.29e-05 & 450 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 0.055 & 97.88 & 0.055 & 97.88 & \textbf{8.49e-05} & 450 & 450 \\
0 & 30 & GT & C2 & 0.055 & \textbf{98.10} & 0.055 & \textbf{98.10} & 8.53e-05 & 450 & 450 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 0.055 & 97.89 & 0.055 & 97.89 & \textbf{8.21e-05} & 450 & 450 \\
0 & 50 & GT & C2 & 0.055 & \textbf{98.11} & 0.055 & \textbf{98.11} & 8.79e-05 & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 0.055 & 97.89 & 0.055 & 97.89 & \textbf{7.85e-05} & 450 & 450 \\
0 & 70 & GT & C2 & 0.055 & \textbf{98.11} & 0.055 & \textbf{98.11} & 8.97e-05 & 450 & 450 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 0.055 & 97.90 & 0.055 & 97.90 & 6.19e-05 & 450 & 450 \\
0 & 100 & GT & C2 & 0.055 & \textbf{98.11} & 0.055 & \textbf{98.11} & \textbf{2.35e-05} & 450 & 450 \\
\addlinespace[1pt]
0 & 30 & N & C1 & 0.055 & 97.88 & 0.055 & 97.88 & \textbf{8.48e-05} & 450 & 450 \\
0 & 30 & N & C2 & 0.055 & \textbf{98.10} & 0.055 & \textbf{98.10} & 8.65e-05 & 450 & 450 \\
\addlinespace[1pt]
0 & 50 & N & C1 & 0.055 & 97.89 & 0.055 & 97.89 & \textbf{8.23e-05} & 450 & 450 \\
0 & 50 & N & C2 & 0.055 & \textbf{98.11} & 0.055 & \textbf{98.11} & 9.20e-05 & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 0.055 & 97.89 & 0.055 & 97.89 & \textbf{7.89e-05} & 450 & 450 \\
0 & 70 & N & C2 & 0.055 & \textbf{98.11} & 0.055 & \textbf{98.11} & 9.44e-05 & 450 & 450 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 0.055 & 97.90 & 0.055 & 97.90 & 6.33e-05 & 450 & 450 \\
0 & 100 & N & C2 & 0.055 & \textbf{98.11} & 0.055 & \textbf{98.11} & \textbf{4.06e-05} & 450 & 450 \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 0.004 & 99.98 & -- & -- & 3.73e-05 & 450 & 0 \\
100 & 100 & GT & C2 & 0.004 & 99.98 & -- & -- & \textbf{1.31e-05} & 450 & 0 \\
\addlinespace[1pt]
100 & 100 & N & C1 & 0.004 & 99.98 & -- & -- & 3.82e-05 & 450 & 0 \\
100 & 100 & N & C2 & 0.004 & 99.98 & -- & -- & \textbf{3.38e-05} & 450 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_c3vd-eval_directed.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, matched-training comparison. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-c3vd-eval-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & \textbf{8.64} & \textbf{29.19} & 71.70 & \textbf{43.95} & \textbf{61.39} \\
0 & 0 & -- & C2 & 7.65 & 27.75 & \textbf{72.20} & 42.70 & 61.27 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & \textbf{6.32} & 25.28 & 59.80 & 36.30 & 54.17 \\
30 & 0 & -- & C2 & 6.17 & \textbf{26.07} & \textbf{60.99} & \textbf{36.45} & \textbf{54.39} \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 7.70 & 30.47 & 63.01 & 39.63 & 56.60 \\
50 & 0 & -- & C2 & \textbf{8.40} & \textbf{30.67} & \textbf{64.30} & \textbf{40.06} & \textbf{56.78} \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 11.31 & \textbf{37.43} & 69.58 & 46.08 & 61.89 \\
70 & 0 & -- & C2 & 11.31 & 36.99 & \textbf{69.83} & \textbf{46.35} & 61.89 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 16.74 & 53.23 & 83.51 & 59.73 & 74.26 \\
100 & 0 & -- & C2 & \textbf{17.04} & \textbf{54.22} & \textbf{84.30} & \textbf{60.13} & \textbf{74.58} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 8.00 & 27.95 & 70.72 & 42.05 & 60.29 \\
0 & 30 & GT & C2 & \textbf{9.68} & \textbf{28.74} & \textbf{70.91} & \textbf{42.19} & \textbf{60.70} \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 8.69 & 28.89 & 71.70 & 43.29 & 61.68 \\
0 & 50 & GT & C2 & \textbf{15.01} & \textbf{35.26} & \textbf{73.14} & \textbf{46.99} & \textbf{64.41} \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 9.23 & 32.25 & 73.88 & 46.28 & 64.36 \\
0 & 70 & GT & C2 & \textbf{25.28} & \textbf{46.81} & \textbf{78.62} & \textbf{56.17} & \textbf{70.91} \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 10.37 & 43.16 & 78.37 & 52.76 & 69.39 \\
0 & 100 & GT & C2 & \textbf{47.90} & \textbf{76.74} & \textbf{95.41} & \textbf{78.63} & \textbf{88.48} \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{7.85} & \textbf{27.60} & \textbf{69.63} & \textbf{41.47} & \textbf{59.40} \\
0 & 30 & N & C2 & 7.26 & 26.02 & 68.25 & 39.70 & 58.35 \\
\addlinespace[1pt]
0 & 50 & N & C1 & 8.30 & 27.95 & \textbf{70.52} & \textbf{42.26} & \textbf{60.22} \\
0 & 50 & N & C2 & \textbf{10.22} & \textbf{28.84} & 67.65 & 40.85 & 58.59 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 9.14 & 31.80 & \textbf{72.40} & \textbf{45.23} & \textbf{62.75} \\
0 & 70 & N & C2 & \textbf{14.81} & \textbf{34.77} & 68.64 & 45.05 & 61.35 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 9.48 & 42.57 & 77.33 & 51.72 & 67.66 \\
0 & 100 & N & C2 & \textbf{29.28} & \textbf{55.46} & \textbf{79.36} & \textbf{60.67} & \textbf{72.75} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 20.74 & 55.51 & 85.14 & 62.26 & 76.34 \\
100 & 100 & GT & C2 & \textbf{56.49} & \textbf{81.78} & \textbf{97.19} & \textbf{82.95} & \textbf{91.04} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 19.85 & 54.07 & \textbf{83.16} & 60.86 & \textbf{74.78} \\
100 & 100 & N & C2 & \textbf{35.16} & \textbf{60.40} & 80.05 & \textbf{63.56} & 74.47 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_c3vd-eval_pose.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, matched-training comparison. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-c3vd-eval-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & 100.00 & 100.00 & 100.00 & \textbf{8.64} & \textbf{29.19} & 71.85 & \textbf{43.97} & \textbf{61.55} \\
0 & 0 & -- & C2 & 100.00 & 100.00 & 100.00 & 7.65 & 27.75 & \textbf{72.30} & 42.73 & 61.49 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 99.95 & 100.00 & 100.00 & \textbf{6.32} & 25.33 & 60.30 & 36.48 & 54.68 \\
30 & 0 & -- & C2 & \textbf{100.00} & 100.00 & 100.00 & 6.17 & \textbf{26.12} & \textbf{61.38} & \textbf{36.58} & \textbf{54.92} \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 100.00 & 100.00 & 100.00 & 7.75 & 30.52 & 63.41 & 39.78 & 57.00 \\
50 & 0 & -- & C2 & 100.00 & 100.00 & 100.00 & \textbf{8.40} & \textbf{30.72} & \textbf{64.69} & \textbf{40.18} & \textbf{57.29} \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 100.00 & 100.00 & 100.00 & 11.31 & \textbf{37.48} & 69.88 & 46.17 & 62.24 \\
70 & 0 & -- & C2 & 100.00 & 100.00 & 100.00 & 11.31 & 36.99 & \textbf{70.12} & \textbf{46.45} & \textbf{62.33} \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 100.00 & 100.00 & 100.00 & 16.74 & 53.23 & 83.51 & 59.73 & 74.26 \\
100 & 0 & -- & C2 & 100.00 & 100.00 & 100.00 & \textbf{17.04} & \textbf{54.22} & \textbf{84.30} & \textbf{60.13} & \textbf{74.59} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 100.00 & 100.00 & 100.00 & 8.00 & 27.95 & 70.81 & 42.07 & 60.43 \\
0 & 30 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{9.68} & \textbf{28.74} & \textbf{71.01} & \textbf{42.23} & \textbf{60.89} \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 100.00 & 100.00 & 100.00 & 8.69 & 28.89 & 71.80 & 43.31 & 61.84 \\
0 & 50 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{15.01} & \textbf{35.26} & \textbf{73.19} & \textbf{46.99} & \textbf{64.52} \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 100.00 & 100.00 & 100.00 & 9.23 & 32.30 & 73.98 & 46.34 & 64.50 \\
0 & 70 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{25.28} & \textbf{46.81} & \textbf{78.67} & \textbf{56.20} & \textbf{71.01} \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 100.00 & 100.00 & 100.00 & 10.37 & 43.16 & 78.37 & 52.76 & 69.42 \\
0 & 100 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{47.90} & \textbf{76.74} & \textbf{95.41} & \textbf{78.63} & \textbf{88.48} \\
\addlinespace[1pt]
0 & 30 & N & C1 & 100.00 & 100.00 & 100.00 & \textbf{7.90} & \textbf{27.65} & \textbf{69.78} & \textbf{41.53} & \textbf{59.62} \\
0 & 30 & N & C2 & 100.00 & 100.00 & 100.00 & 7.26 & 26.02 & 68.44 & 39.77 & 58.60 \\
\addlinespace[1pt]
0 & 50 & N & C1 & 100.00 & 100.00 & 100.00 & 8.30 & 28.00 & \textbf{70.62} & \textbf{42.30} & \textbf{60.38} \\
0 & 50 & N & C2 & 100.00 & 100.00 & 100.00 & \textbf{10.22} & \textbf{28.84} & 67.75 & 40.87 & 58.77 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 100.00 & 100.00 & 100.00 & 9.19 & 31.85 & \textbf{72.49} & \textbf{45.31} & \textbf{62.94} \\
0 & 70 & N & C2 & 100.00 & 100.00 & 100.00 & \textbf{14.81} & \textbf{34.77} & 68.69 & 45.06 & 61.50 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 100.00 & 100.00 & 100.00 & 9.48 & 42.62 & 77.38 & 51.77 & 67.73 \\
0 & 100 & N & C2 & 100.00 & 100.00 & 100.00 & \textbf{29.28} & \textbf{55.46} & \textbf{79.46} & \textbf{60.70} & \textbf{72.81} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 100.00 & 100.00 & 100.00 & 20.74 & 55.51 & 85.19 & 62.26 & 76.36 \\
100 & 100 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{56.49} & \textbf{81.78} & \textbf{97.19} & \textbf{82.95} & \textbf{91.04} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 100.00 & 100.00 & 100.00 & 19.85 & 54.07 & \textbf{83.16} & 60.86 & \textbf{74.80} \\
100 & 100 & N & C2 & 100.00 & 100.00 & 100.00 & \textbf{35.16} & \textbf{60.40} & 80.15 & \textbf{63.58} & 74.53 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_c3vd-eval_retention.tex <==
\begin{table}[tbp]
\centering
\caption{C3VD, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:trained-c3vd-eval-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 135 & 135 \\
0 & 30 & GT & C1 & 100.00 & 100.00 & 7.41 & 37.04 & 49.53 & 69.70 & 135 & 135 \\
0 & 30 & GT & C2 & 100.00 & 100.00 & 49.63 & 79.26 & 81.53 & 90.57 & 135 & 135 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 450 & 450 \\
0 & 50 & GT & C1 & 100.00 & 100.00 & 11.56 & 38.00 & 49.87 & 68.90 & 450 & 450 \\
0 & 50 & GT & C2 & 100.00 & 100.00 & 44.44 & 80.00 & 80.80 & 89.86 & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 945 & 945 \\
0 & 70 & GT & C1 & 100.00 & 100.00 & 11.53 & 39.37 & 51.15 & 69.35 & 945 & 945 \\
0 & 70 & GT & C2 & 100.00 & 100.00 & 46.98 & 78.20 & 80.68 & 89.65 & 945 & 945 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 2025 & 2025 \\
0 & 100 & GT & C1 & 100.00 & 100.00 & 10.37 & 43.16 & 52.76 & 69.42 & 2025 & 2025 \\
0 & 100 & GT & C2 & 100.00 & 100.00 & 47.90 & 76.74 & 78.63 & 88.48 & 2025 & 2025 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 17.04 & 43.70 & 47.85 & 59.43 & 135 & 135 \\
0 & 30 & N & C1 & 100.00 & 100.00 & 7.41 & 30.37 & 43.11 & 58.86 & 135 & 135 \\
0 & 30 & N & C2 & 100.00 & 100.00 & 17.78 & 45.93 & 50.52 & 61.70 & 135 & 135 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 26.67 & 49.78 & 52.47 & 63.66 & 450 & 450 \\
0 & 50 & N & C1 & 100.00 & 100.00 & 9.56 & 34.67 & 45.61 & 63.04 & 450 & 450 \\
0 & 50 & N & C2 & 100.00 & 100.00 & 24.00 & 51.33 & 55.53 & 67.07 & 450 & 450 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 31.43 & 52.80 & 56.59 & 67.76 & 945 & 945 \\
0 & 70 & N & C1 & 100.00 & 100.00 & 11.11 & 37.88 & 49.02 & 66.02 & 945 & 945 \\
0 & 70 & N & C2 & 100.00 & 100.00 & 24.87 & 51.96 & 57.20 & 69.80 & 945 & 945 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 100.00 & 100.00 & 37.28 & 57.73 & 61.36 & 71.73 & 2025 & 2025 \\
0 & 100 & N & C1 & 100.00 & 100.00 & 9.48 & 42.62 & 51.77 & 67.73 & 2025 & 2025 \\
0 & 100 & N & C2 & 100.00 & 100.00 & 29.28 & 55.46 & 60.70 & 72.81 & 2025 & 2025 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 2025 & 2025 \\
100 & 100 & GT & C1 & 100.00 & 100.00 & 20.74 & 55.51 & 62.26 & 76.36 & 2025 & 2025 \\
100 & 100 & GT & C2 & 100.00 & 100.00 & 56.49 & 81.78 & 82.95 & 91.04 & 2025 & 2025 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 100.00 & 100.00 & 37.28 & 57.73 & 61.36 & 71.73 & 2025 & 2025 \\
100 & 100 & N & C1 & 100.00 & 100.00 & 19.85 & 54.07 & 60.86 & 74.80 & 2025 & 2025 \\
100 & 100 & N & C2 & 100.00 & 100.00 & 35.16 & 60.40 & 63.58 & 74.53 & 2025 & 2025 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_tum-eval_depth.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, matched-training comparison. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-tum-eval-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & C1 & 0.058 & \textbf{94.64} & 0.058 & \textbf{94.64} & 4.56e-03 & 200 & 200 \\
0 & 0 & -- & C2 & 0.058 & 94.41 & 0.058 & 94.41 & \textbf{4.54e-03} & 200 & 200 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 0.031 & \textbf{98.05} & 0.040 & \textbf{97.32} & 5.38e-03 & 200 & 140 \\
30 & 0 & -- & C2 & 0.031 & 98.04 & 0.040 & 97.31 & \textbf{5.33e-03} & 200 & 140 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 0.024 & \textbf{98.58} & 0.038 & \textbf{97.40} & \textbf{5.19e-03} & 200 & 100 \\
50 & 0 & -- & C2 & \textbf{0.023} & 98.57 & \textbf{0.037} & 97.39 & 5.21e-03 & 200 & 100 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 0.017 & 99.11 & 0.034 & 97.62 & 4.89e-03 & 200 & 60 \\
70 & 0 & -- & C2 & \textbf{0.016} & 99.11 & \textbf{0.033} & 97.62 & \textbf{4.74e-03} & 200 & 60 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 0.009 & 99.76 & -- & -- & 4.45e-03 & 200 & 0 \\
100 & 0 & -- & C2 & 0.009 & 99.76 & -- & -- & \textbf{4.26e-03} & 200 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & C1 & \textbf{0.057} & \textbf{94.66} & \textbf{0.057} & \textbf{94.66} & 4.62e-03 & 200 & 200 \\
0 & 30 & GT & C2 & 0.058 & 94.44 & 0.058 & 94.44 & \textbf{4.36e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & \textbf{0.057} & \textbf{94.68} & \textbf{0.057} & \textbf{94.68} & 4.68e-03 & 200 & 200 \\
0 & 50 & GT & C2 & 0.058 & 94.46 & 0.058 & 94.46 & \textbf{4.06e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & \textbf{0.057} & \textbf{94.69} & \textbf{0.057} & \textbf{94.69} & 4.82e-03 & 200 & 200 \\
0 & 70 & GT & C2 & 0.058 & 94.46 & 0.058 & 94.46 & \textbf{4.11e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & \textbf{0.057} & \textbf{94.69} & \textbf{0.057} & \textbf{94.69} & 3.38e-03 & 200 & 200 \\
0 & 100 & GT & C2 & 0.058 & 94.49 & 0.058 & 94.49 & \textbf{2.16e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{0.057} & \textbf{94.66} & \textbf{0.057} & \textbf{94.66} & 4.64e-03 & 200 & 200 \\
0 & 30 & N & C2 & 0.058 & 94.44 & 0.058 & 94.44 & \textbf{4.42e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 50 & N & C1 & \textbf{0.057} & \textbf{94.68} & \textbf{0.057} & \textbf{94.68} & 4.73e-03 & 200 & 200 \\
0 & 50 & N & C2 & 0.058 & 94.46 & 0.058 & 94.46 & \textbf{4.26e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & N & C1 & \textbf{0.057} & \textbf{94.69} & \textbf{0.057} & \textbf{94.69} & 4.84e-03 & 200 & 200 \\
0 & 70 & N & C2 & 0.058 & 94.46 & 0.058 & 94.46 & \textbf{4.39e-03} & 200 & 200 \\
\addlinespace[1pt]
0 & 100 & N & C1 & \textbf{0.057} & \textbf{94.70} & \textbf{0.057} & \textbf{94.70} & 3.40e-03 & 200 & 200 \\
0 & 100 & N & C2 & 0.058 & 94.51 & 0.058 & 94.51 & \textbf{2.45e-03} & 200 & 200 \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 0.009 & 99.76 & -- & -- & 3.59e-03 & 200 & 0 \\
100 & 100 & GT & C2 & 0.009 & 99.76 & -- & -- & \textbf{2.07e-03} & 200 & 0 \\
\addlinespace[1pt]
100 & 100 & N & C1 & 0.009 & 99.76 & -- & -- & 3.54e-03 & 200 & 0 \\
100 & 100 & N & C2 & 0.009 & 99.76 & -- & -- & \textbf{2.26e-03} & 200 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_tum-eval_directed.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, matched-training comparison. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-tum-eval-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & \textbf{22.22} & \textbf{51.22} & 75.67 & \textbf{56.73} & 69.09 \\
0 & 0 & -- & C2 & 20.22 & 50.33 & \textbf{76.44} & 56.50 & \textbf{69.17} \\
\addlinespace[1pt]
30 & 0 & -- & C1 & \textbf{17.44} & 47.33 & 72.78 & 52.84 & 66.23 \\
30 & 0 & -- & C2 & 17.11 & \textbf{48.56} & \textbf{73.44} & \textbf{52.90} & \textbf{66.56} \\
\addlinespace[1pt]
50 & 0 & -- & C1 & \textbf{17.11} & 45.78 & \textbf{73.44} & \textbf{52.42} & 66.00 \\
50 & 0 & -- & C2 & 16.56 & \textbf{45.89} & 73.22 & 52.10 & \textbf{66.39} \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 19.11 & 47.89 & 75.33 & 54.75 & 67.91 \\
70 & 0 & -- & C2 & 19.11 & \textbf{49.22} & \textbf{76.67} & \textbf{55.39} & \textbf{68.66} \\
\addlinespace[1pt]
100 & 0 & -- & C1 & \textbf{27.22} & 51.89 & 78.00 & 58.50 & 70.58 \\
100 & 0 & -- & C2 & 26.00 & \textbf{52.33} & \textbf{79.33} & \textbf{59.19} & \textbf{71.65} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 19.11 & 49.00 & 75.33 & 55.01 & 67.88 \\
0 & 30 & GT & C2 & \textbf{20.33} & \textbf{51.00} & \textbf{76.33} & \textbf{56.64} & \textbf{69.21} \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 16.89 & 49.67 & 74.44 & 54.41 & 67.17 \\
0 & 50 & GT & C2 & \textbf{24.00} & \textbf{55.00} & \textbf{77.67} & \textbf{58.95} & \textbf{70.63} \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 19.22 & 51.56 & 75.44 & 56.14 & 68.19 \\
0 & 70 & GT & C2 & \textbf{31.56} & \textbf{60.11} & \textbf{80.22} & \textbf{62.79} & \textbf{73.49} \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 25.11 & 58.78 & 77.56 & 60.35 & 71.04 \\
0 & 100 & GT & C2 & \textbf{52.00} & \textbf{73.78} & \textbf{84.00} & \textbf{72.22} & \textbf{80.46} \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{18.67} & 49.22 & 74.67 & 54.95 & 67.81 \\
0 & 30 & N & C2 & 18.33 & \textbf{49.78} & \textbf{75.67} & \textbf{55.70} & \textbf{68.53} \\
\addlinespace[1pt]
0 & 50 & N & C1 & 16.22 & 49.11 & 74.56 & 54.08 & 66.98 \\
0 & 50 & N & C2 & \textbf{20.11} & \textbf{51.11} & \textbf{76.78} & \textbf{56.81} & \textbf{69.21} \\
\addlinespace[1pt]
0 & 70 & N & C1 & 19.67 & 51.44 & 75.22 & 56.22 & 68.19 \\
0 & 70 & N & C2 & \textbf{22.56} & \textbf{55.00} & \textbf{78.11} & \textbf{58.86} & \textbf{70.87} \\
\addlinespace[1pt]
0 & 100 & N & C1 & 27.22 & 58.89 & 76.11 & 60.44 & 70.89 \\
0 & 100 & N & C2 & \textbf{35.33} & \textbf{67.00} & \textbf{81.44} & \textbf{66.07} & \textbf{76.37} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 27.89 & 55.89 & 78.00 & 59.99 & 71.81 \\
100 & 100 & GT & C2 & \textbf{41.78} & \textbf{68.44} & \textbf{84.78} & \textbf{68.91} & \textbf{79.08} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 27.33 & 55.56 & 78.56 & 59.01 & 71.13 \\
100 & 100 & N & C2 & \textbf{27.78} & \textbf{63.44} & \textbf{82.11} & \textbf{63.78} & \textbf{75.31} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_tum-eval_pose.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, matched-training comparison. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-tum-eval-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & 94.78 & 96.33 & 97.22 & \textbf{22.22} & \textbf{51.22} & 75.78 & \textbf{56.78} & 69.17 \\
0 & 0 & -- & C2 & \textbf{95.44} & \textbf{97.22} & 97.22 & 20.22 & 50.33 & \textbf{76.56} & 56.53 & \textbf{69.33} \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 94.11 & 97.00 & 97.22 & \textbf{17.44} & 47.33 & 73.00 & 52.87 & 66.46 \\
30 & 0 & -- & C2 & \textbf{96.56} & \textbf{97.22} & 97.22 & 17.11 & \textbf{48.56} & \textbf{73.44} & \textbf{52.90} & \textbf{66.66} \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 94.78 & 95.56 & 97.22 & \textbf{17.11} & 45.78 & \textbf{73.56} & \textbf{52.44} & 66.21 \\
50 & 0 & -- & C2 & \textbf{96.89} & \textbf{97.22} & 97.22 & 16.56 & \textbf{45.89} & 73.33 & 52.10 & \textbf{66.46} \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 94.33 & 95.33 & 97.00 & 19.11 & 47.89 & 75.56 & 54.80 & 68.22 \\
70 & 0 & -- & C2 & \textbf{95.44} & \textbf{97.22} & \textbf{97.22} & 19.11 & \textbf{49.22} & \textbf{76.78} & \textbf{55.41} & \textbf{68.87} \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 93.56 & 95.44 & 95.44 & \textbf{27.22} & 51.89 & 78.11 & 58.50 & 70.71 \\
100 & 0 & -- & C2 & \textbf{95.89} & \textbf{96.22} & \textbf{97.22} & 26.00 & \textbf{52.33} & \textbf{79.44} & \textbf{59.19} & \textbf{71.77} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 95.00 & 96.44 & 97.22 & 19.11 & 49.00 & 75.33 & 55.01 & 67.92 \\
0 & 30 & GT & C2 & \textbf{95.67} & \textbf{97.22} & 97.22 & \textbf{20.33} & \textbf{51.00} & \textbf{76.33} & \textbf{56.64} & \textbf{69.29} \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 95.11 & 96.44 & 97.22 & 16.89 & 49.67 & 74.44 & 54.41 & 67.19 \\
0 & 50 & GT & C2 & \textbf{95.67} & \textbf{97.22} & 97.22 & \textbf{24.00} & \textbf{55.00} & \textbf{77.89} & \textbf{58.95} & \textbf{70.74} \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 95.11 & 96.11 & 96.56 & 19.22 & 51.56 & 75.56 & 56.17 & 68.26 \\
0 & 70 & GT & C2 & \textbf{95.44} & \textbf{96.56} & \textbf{97.67} & \textbf{31.56} & \textbf{60.11} & \textbf{80.22} & \textbf{62.79} & \textbf{73.50} \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 96.22 & \textbf{97.22} & 97.22 & 25.11 & 58.78 & 77.56 & 60.35 & 71.04 \\
0 & 100 & GT & C2 & \textbf{96.44} & 96.89 & \textbf{98.89} & \textbf{52.00} & \textbf{73.78} & \textbf{84.00} & \textbf{72.22} & \textbf{80.46} \\
\addlinespace[1pt]
0 & 30 & N & C1 & 95.00 & 96.44 & 97.22 & \textbf{18.67} & 49.22 & 74.67 & 54.95 & 67.85 \\
0 & 30 & N & C2 & \textbf{95.56} & \textbf{97.22} & 97.22 & 18.33 & \textbf{49.78} & \textbf{75.67} & \textbf{55.70} & \textbf{68.64} \\
\addlinespace[1pt]
0 & 50 & N & C1 & 95.11 & 96.44 & 97.22 & 16.22 & 49.11 & 74.56 & 54.08 & 67.00 \\
0 & 50 & N & C2 & \textbf{95.67} & \textbf{97.22} & 97.22 & \textbf{20.11} & \textbf{51.11} & \textbf{77.00} & \textbf{56.81} & \textbf{69.28} \\
\addlinespace[1pt]
0 & 70 & N & C1 & 95.11 & 96.11 & 96.56 & 19.67 & 51.44 & 75.56 & 56.23 & 68.25 \\
0 & 70 & N & C2 & \textbf{95.44} & \textbf{96.56} & \textbf{97.67} & \textbf{22.56} & \textbf{55.00} & \textbf{78.11} & \textbf{58.86} & \textbf{70.89} \\
\addlinespace[1pt]
0 & 100 & N & C1 & 96.11 & 97.22 & 97.22 & 27.22 & 58.89 & 76.11 & 60.44 & 70.89 \\
0 & 100 & N & C2 & \textbf{96.78} & 97.22 & \textbf{98.89} & \textbf{35.33} & \textbf{67.00} & \textbf{81.44} & \textbf{66.07} & \textbf{76.37} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 94.89 & 95.44 & 95.44 & 27.89 & 55.89 & 78.00 & 59.99 & 71.86 \\
100 & 100 & GT & C2 & \textbf{95.33} & \textbf{96.56} & \textbf{97.22} & \textbf{41.78} & \textbf{68.44} & \textbf{84.78} & \textbf{68.91} & \textbf{79.08} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 94.78 & 95.44 & 95.44 & 27.33 & 55.56 & 78.56 & 59.01 & 71.16 \\
100 & 100 & N & C2 & \textbf{95.22} & \textbf{96.67} & \textbf{97.22} & \textbf{27.78} & \textbf{63.44} & \textbf{82.11} & \textbf{63.78} & \textbf{75.31} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_tum-eval_retention.tex <==
\begin{table}[tbp]
\centering
\caption{TUM RGB-D, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:trained-tum-eval-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 60 & 60 \\
0 & 30 & GT & C1 & 100.00 & 100.00 & 3.33 & 35.00 & 50.78 & 67.56 & 60 & 60 \\
0 & 30 & GT & C2 & 100.00 & 100.00 & 40.00 & 76.67 & 74.22 & 82.78 & 60 & 60 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 200 & 200 \\
0 & 50 & GT & C1 & 100.00 & 100.00 & 12.00 & 49.50 & 55.20 & 68.23 & 200 & 200 \\
0 & 50 & GT & C2 & 100.00 & 100.00 & 46.50 & 73.50 & 71.70 & 79.90 & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 420 & 420 \\
0 & 70 & GT & C1 & 97.38 & 97.62 & 21.43 & 54.52 & 59.06 & 71.29 & 420 & 420 \\
0 & 70 & GT & C2 & 97.62 & 97.62 & 48.81 & 72.62 & 72.87 & 81.03 & 420 & 420 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 900 & 900 \\
0 & 100 & GT & C1 & 96.22 & 97.22 & 25.11 & 58.78 & 60.35 & 71.04 & 900 & 900 \\
0 & 100 & GT & C2 & 96.44 & 96.89 & 52.00 & 73.78 & 72.22 & 80.46 & 900 & 900 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 21.67 & 63.33 & 65.78 & 80.56 & 60 & 60 \\
0 & 30 & N & C1 & 100.00 & 100.00 & 1.67 & 33.33 & 49.22 & 66.28 & 60 & 60 \\
0 & 30 & N & C2 & 100.00 & 100.00 & 16.67 & 65.00 & 64.67 & 75.78 & 60 & 60 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 24.00 & 64.50 & 68.97 & 83.52 & 200 & 200 \\
0 & 50 & N & C1 & 100.00 & 100.00 & 11.50 & 48.50 & 54.53 & 68.25 & 200 & 200 \\
0 & 50 & N & C2 & 100.00 & 100.00 & 29.50 & 63.00 & 64.90 & 75.68 & 200 & 200 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 26.19 & 65.71 & 68.27 & 82.75 & 420 & 420 \\
0 & 70 & N & C1 & 97.38 & 97.62 & 22.38 & 55.00 & 59.65 & 71.46 & 420 & 420 \\
0 & 70 & N & C2 & 97.62 & 97.62 & 30.95 & 65.00 & 66.62 & 76.81 & 420 & 420 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 100.00 & 100.00 & 26.44 & 66.00 & 67.87 & 81.07 & 900 & 900 \\
0 & 100 & N & C1 & 96.11 & 97.22 & 27.22 & 58.89 & 60.44 & 70.89 & 900 & 900 \\
0 & 100 & N & C2 & 96.78 & 97.22 & 35.33 & 67.00 & 66.07 & 76.37 & 900 & 900 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 900 & 900 \\
100 & 100 & GT & C1 & 94.89 & 95.44 & 27.89 & 55.89 & 59.99 & 71.86 & 900 & 900 \\
100 & 100 & GT & C2 & 95.33 & 96.56 & 41.78 & 68.44 & 68.91 & 79.08 & 900 & 900 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 100.00 & 100.00 & 26.44 & 66.00 & 67.87 & 81.07 & 900 & 900 \\
100 & 100 & N & C1 & 94.78 & 95.44 & 27.33 & 55.56 & 59.01 & 71.16 & 900 & 900 \\
100 & 100 & N & C2 & 95.22 & 96.67 & 27.78 & 63.44 & 63.78 & 75.31 & 900 & 900 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_v2_depth.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, matched-training comparison. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-v2-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & C1 & 0.109 & \textbf{89.62} & 0.109 & \textbf{89.62} & \textbf{2.72e-01} & 6600 & 6600 \\
0 & 0 & -- & C2 & 0.109 & 89.59 & 0.109 & 89.59 & 2.91e-01 & 6600 & 6600 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 0.065 & \textbf{94.00} & \textbf{0.084} & \textbf{91.86} & \textbf{2.92e-01} & 6600 & 4620 \\
30 & 0 & -- & C2 & 0.065 & 93.95 & 0.085 & 91.78 & 2.95e-01 & 6600 & 4620 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 0.050 & \textbf{95.58} & \textbf{0.080} & \textbf{92.15} & \textbf{3.05e-01} & 6600 & 3300 \\
50 & 0 & -- & C2 & 0.050 & 95.56 & 0.081 & 92.10 & 3.06e-01 & 6600 & 3300 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 0.037 & \textbf{97.14} & 0.075 & \textbf{92.77} & 3.15e-01 & 6600 & 1980 \\
70 & 0 & -- & C2 & 0.037 & 97.12 & 0.075 & 92.69 & \textbf{3.09e-01} & 6600 & 1980 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 0.021 & 99.00 & -- & -- & 3.04e-01 & 6600 & 0 \\
100 & 0 & -- & C2 & 0.021 & \textbf{99.01} & -- & -- & \textbf{2.97e-01} & 6600 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & C1 & \textbf{0.108} & \textbf{89.70} & \textbf{0.108} & \textbf{89.70} & \textbf{3.01e-01} & 6600 & 6600 \\
0 & 30 & GT & C2 & 0.109 & 89.65 & 0.109 & 89.65 & 3.40e-01 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 0.108 & \textbf{89.75} & 0.108 & \textbf{89.75} & \textbf{2.95e-01} & 6600 & 6600 \\
0 & 50 & GT & C2 & 0.108 & 89.70 & 0.108 & 89.70 & 3.28e-01 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & \textbf{0.107} & \textbf{89.79} & \textbf{0.107} & \textbf{89.79} & \textbf{2.78e-01} & 6600 & 6600 \\
0 & 70 & GT & C2 & 0.108 & 89.75 & 0.108 & 89.75 & 3.10e-01 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 0.107 & \textbf{89.88} & 0.107 & \textbf{89.88} & 1.50e-01 & 6600 & 6600 \\
0 & 100 & GT & C2 & 0.107 & 89.83 & 0.107 & 89.83 & \textbf{1.48e-01} & 6600 & 6600 \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{0.108} & \textbf{89.70} & \textbf{0.108} & \textbf{89.70} & \textbf{3.01e-01} & 6600 & 6600 \\
0 & 30 & N & C2 & 0.109 & 89.65 & 0.109 & 89.65 & 3.40e-01 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 50 & N & C1 & 0.108 & \textbf{89.75} & 0.108 & \textbf{89.75} & \textbf{2.95e-01} & 6600 & 6600 \\
0 & 50 & N & C2 & 0.108 & 89.71 & 0.108 & 89.71 & 3.29e-01 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & N & C1 & \textbf{0.107} & \textbf{89.79} & \textbf{0.107} & \textbf{89.79} & \textbf{2.79e-01} & 6600 & 6600 \\
0 & 70 & N & C2 & 0.108 & 89.75 & 0.108 & 89.75 & 3.10e-01 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 0.107 & \textbf{89.88} & 0.107 & \textbf{89.88} & 1.49e-01 & 6600 & 6600 \\
0 & 100 & N & C2 & 0.107 & 89.83 & 0.107 & 89.83 & 1.49e-01 & 6600 & 6600 \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 0.020 & 99.01 & -- & -- & 1.41e-01 & 6600 & 0 \\
100 & 100 & GT & C2 & 0.020 & 99.01 & -- & -- & \textbf{1.38e-01} & 6600 & 0 \\
\addlinespace[1pt]
100 & 100 & N & C1 & 0.020 & 99.01 & -- & -- & 1.41e-01 & 6600 & 0 \\
100 & 100 & N & C2 & 0.020 & 99.01 & -- & -- & \textbf{1.39e-01} & 6600 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_v2_directed.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, matched-training comparison. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-v2-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & 10.48 & \textbf{46.43} & \textbf{87.99} & \textbf{57.97} & \textbf{74.81} \\
0 & 0 & -- & C2 & \textbf{10.69} & 46.30 & 87.46 & 57.68 & 74.41 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 9.29 & \textbf{42.11} & \textbf{86.41} & \textbf{55.68} & \textbf{73.15} \\
30 & 0 & -- & C2 & \textbf{9.31} & 41.92 & 86.08 & 55.39 & 72.88 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & \textbf{9.03} & \textbf{41.77} & \textbf{85.92} & \textbf{55.38} & \textbf{72.78} \\
50 & 0 & -- & C2 & 8.98 & 41.56 & 85.44 & 55.01 & 72.49 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & \textbf{8.84} & \textbf{41.17} & \textbf{85.88} & \textbf{55.29} & \textbf{72.60} \\
70 & 0 & -- & C2 & 8.47 & 40.65 & 85.55 & 54.93 & 72.37 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & \textbf{8.32} & \textbf{40.77} & 86.17 & \textbf{55.39} & 72.73 \\
100 & 0 & -- & C2 & 8.13 & 40.33 & \textbf{86.29} & 55.21 & \textbf{72.77} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & \textbf{12.13} & \textbf{46.23} & \textbf{84.64} & \textbf{55.75} & \textbf{72.71} \\
0 & 30 & GT & C2 & 11.45 & 43.76 & 82.20 & 53.51 & 70.68 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & \textbf{13.85} & \textbf{49.54} & \textbf{85.42} & \textbf{57.41} & \textbf{73.84} \\
0 & 50 & GT & C2 & 13.72 & 46.92 & 82.97 & 55.03 & 71.78 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 17.68 & \textbf{57.00} & \textbf{87.62} & \textbf{61.84} & \textbf{76.69} \\
0 & 70 & GT & C2 & \textbf{18.78} & 55.51 & 85.86 & 60.46 & 75.46 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 25.89 & 73.32 & 94.18 & 73.08 & 84.65 \\
0 & 100 & GT & C2 & \textbf{31.41} & \textbf{76.65} & \textbf{94.32} & \textbf{75.32} & \textbf{85.82} \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{12.11} & \textbf{46.26} & \textbf{84.65} & \textbf{55.73} & \textbf{72.70} \\
0 & 30 & N & C2 & 11.48 & 43.63 & 82.22 & 53.47 & 70.65 \\
\addlinespace[1pt]
0 & 50 & N & C1 & \textbf{13.86} & \textbf{49.57} & \textbf{85.40} & \textbf{57.39} & \textbf{73.82} \\
0 & 50 & N & C2 & 13.55 & 46.79 & 82.94 & 54.93 & 71.72 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 17.65 & \textbf{57.05} & \textbf{87.63} & \textbf{61.82} & \textbf{76.67} \\
0 & 70 & N & C2 & \textbf{18.18} & 55.25 & 85.76 & 60.24 & 75.33 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 25.94 & 73.12 & 94.17 & 73.06 & 84.64 \\
0 & 100 & N & C2 & \textbf{29.32} & \textbf{75.76} & \textbf{94.21} & \textbf{74.64} & \textbf{85.47} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 24.08 & 74.66 & 93.99 & 73.33 & 84.70 \\
100 & 100 & GT & C2 & \textbf{27.59} & \textbf{76.87} & \textbf{94.58} & \textbf{74.98} & \textbf{85.76} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 23.86 & 74.65 & 93.98 & 73.29 & 84.66 \\
100 & 100 & N & C2 & \textbf{25.99} & \textbf{76.05} & \textbf{94.53} & \textbf{74.43} & \textbf{85.47} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_v2_pose.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, matched-training comparison. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-v2-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & 58.52 & \textbf{88.69} & \textbf{96.46} & 10.49 & \textbf{46.48} & \textbf{88.31} & \textbf{58.07} & \textbf{75.01} \\
0 & 0 & -- & C2 & \textbf{58.97} & 88.37 & 96.12 & \textbf{10.69} & 46.35 & 87.78 & 57.77 & 74.63 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & \textbf{60.92} & \textbf{88.91} & \textbf{96.28} & 9.30 & \textbf{42.18} & \textbf{86.72} & \textbf{55.78} & \textbf{73.39} \\
30 & 0 & -- & C2 & 60.56 & 88.48 & 96.24 & \textbf{9.32} & 41.98 & 86.39 & 55.50 & 73.12 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & \textbf{62.41} & \textbf{89.00} & \textbf{96.03} & \textbf{9.04} & \textbf{41.86} & \textbf{86.26} & \textbf{55.49} & \textbf{73.01} \\
50 & 0 & -- & C2 & 62.32 & 88.78 & 95.96 & 8.99 & 41.66 & 85.77 & 55.12 & 72.77 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & \textbf{64.55} & \textbf{89.48} & 96.00 & \textbf{8.87} & \textbf{41.28} & \textbf{86.35} & \textbf{55.42} & \textbf{72.90} \\
70 & 0 & -- & C2 & 64.30 & 89.34 & \textbf{96.11} & 8.48 & 40.72 & 85.92 & 55.07 & 72.67 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 67.02 & 90.17 & \textbf{96.12} & \textbf{8.33} & \textbf{40.87} & 86.62 & \textbf{55.53} & 73.01 \\
100 & 0 & -- & C2 & \textbf{67.26} & \textbf{90.32} & 96.03 & 8.14 & 40.40 & \textbf{86.64} & 55.34 & \textbf{73.04} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & \textbf{62.22} & \textbf{89.37} & \textbf{96.46} & \textbf{12.13} & \textbf{46.28} & \textbf{84.95} & \textbf{55.86} & \textbf{72.91} \\
0 & 30 & GT & C2 & 62.05 & 89.13 & 96.28 & 11.46 & 43.81 & 82.52 & 53.62 & 70.92 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & \textbf{64.34} & \textbf{89.81} & \textbf{96.61} & \textbf{13.86} & \textbf{49.60} & \textbf{85.73} & \textbf{57.51} & \textbf{74.03} \\
0 & 50 & GT & C2 & 64.31 & 89.48 & 96.59 & 13.72 & 46.96 & 83.26 & 55.14 & 72.00 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 69.40 & \textbf{91.25} & \textbf{97.14} & 17.68 & \textbf{57.03} & \textbf{87.90} & \textbf{61.93} & \textbf{76.87} \\
0 & 70 & GT & C2 & \textbf{70.03} & 91.03 & 97.02 & \textbf{18.79} & 55.55 & 86.12 & 60.54 & 75.65 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 85.50 & 95.83 & 98.36 & 25.89 & 73.32 & 94.21 & 73.09 & 84.67 \\
0 & 100 & GT & C2 & \textbf{88.55} & \textbf{95.85} & \textbf{98.49} & \textbf{31.41} & \textbf{76.65} & \textbf{94.34} & \textbf{75.33} & \textbf{85.85} \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{62.22} & \textbf{89.37} & \textbf{96.46} & \textbf{12.11} & \textbf{46.31} & \textbf{84.94} & \textbf{55.83} & \textbf{72.90} \\
0 & 30 & N & C2 & 62.10 & 89.11 & 96.29 & 11.49 & 43.68 & 82.54 & 53.57 & 70.89 \\
\addlinespace[1pt]
0 & 50 & N & C1 & \textbf{64.27} & \textbf{89.81} & \textbf{96.61} & \textbf{13.87} & \textbf{49.63} & \textbf{85.71} & \textbf{57.49} & \textbf{74.02} \\
0 & 50 & N & C2 & 64.18 & 89.47 & 96.59 & 13.55 & 46.83 & 83.24 & 55.04 & 71.94 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 69.21 & \textbf{91.26} & \textbf{97.14} & 17.65 & \textbf{57.08} & \textbf{87.91} & \textbf{61.91} & \textbf{76.86} \\
0 & 70 & N & C2 & \textbf{69.82} & 91.02 & 97.01 & \textbf{18.19} & 55.28 & 86.03 & 60.32 & 75.52 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 85.37 & \textbf{95.82} & 98.34 & 25.94 & 73.12 & 94.20 & 73.06 & 84.65 \\
0 & 100 & N & C2 & \textbf{87.89} & 95.81 & \textbf{98.47} & \textbf{29.32} & \textbf{75.77} & \textbf{94.24} & \textbf{74.65} & \textbf{85.50} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 87.33 & 95.87 & 98.13 & 24.08 & 74.66 & 94.06 & 73.36 & 84.76 \\
100 & 100 & GT & C2 & \textbf{90.59} & \textbf{96.42} & \textbf{98.68} & \textbf{27.59} & \textbf{76.87} & \textbf{94.60} & \textbf{74.99} & \textbf{85.80} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 87.06 & 95.86 & 98.14 & 23.86 & 74.65 & 94.05 & 73.31 & 84.72 \\
100 & 100 & N & C2 & \textbf{89.89} & \textbf{96.39} & \textbf{98.70} & \textbf{25.99} & \textbf{76.05} & \textbf{94.56} & \textbf{74.44} & \textbf{85.51} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_v2_retention.tex <==
\begin{table}[tbp]
\centering
\caption{TartanAir-V2, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:trained-v2-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 1980 & 1980 \\
0 & 30 & GT & C1 & 96.31 & 98.84 & 18.74 & 63.69 & 68.53 & 82.40 & 1980 & 1980 \\
0 & 30 & GT & C2 & 97.02 & 99.19 & 22.98 & 64.19 & 69.69 & 83.04 & 1980 & 1980 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 6600 & 6600 \\
0 & 50 & GT & C1 & 93.23 & 98.05 & 21.44 & 69.64 & 71.35 & 83.91 & 6600 & 6600 \\
0 & 50 & GT & C2 & 94.24 & 98.17 & 25.55 & 72.05 & 73.14 & 85.03 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 13860 & 13860 \\
0 & 70 & GT & C1 & 90.10 & 97.39 & 23.83 & 71.75 & 72.64 & 84.67 & 13860 & 13860 \\
0 & 70 & GT & C2 & 91.80 & 97.59 & 27.91 & 74.63 & 74.62 & 85.86 & 13860 & 13860 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 29700 & 29700 \\
0 & 100 & GT & C1 & 85.50 & 95.83 & 25.89 & 73.32 & 73.09 & 84.67 & 29700 & 29700 \\
0 & 100 & GT & C2 & 88.55 & 95.85 & 31.41 & 76.65 & 75.33 & 85.85 & 29700 & 29700 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 49.39 & 82.93 & 82.16 & 90.67 & 1980 & 1980 \\
0 & 30 & N & C1 & 96.21 & 98.84 & 18.54 & 63.79 & 68.39 & 82.35 & 1980 & 1980 \\
0 & 30 & N & C2 & 97.07 & 99.19 & 23.08 & 63.23 & 69.28 & 82.76 & 1980 & 1980 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 48.68 & 83.64 & 82.60 & 90.97 & 6600 & 6600 \\
0 & 50 & N & C1 & 93.12 & 98.09 & 21.55 & 69.77 & 71.34 & 83.89 & 6600 & 6600 \\
0 & 50 & N & C2 & 94.00 & 98.15 & 24.70 & 71.36 & 72.79 & 84.83 & 6600 & 6600 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 47.98 & 83.95 & 82.69 & 91.00 & 13860 & 13860 \\
0 & 70 & N & C1 & 89.98 & 97.40 & 23.85 & 71.85 & 72.62 & 84.65 & 13860 & 13860 \\
0 & 70 & N & C2 & 91.52 & 97.53 & 26.76 & 74.30 & 74.25 & 85.64 & 13860 & 13860 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 99.85 & 100.00 & 47.41 & 84.00 & 82.72 & 91.01 & 29700 & 29700 \\
0 & 100 & N & C1 & 85.37 & 95.82 & 25.94 & 73.12 & 73.06 & 84.65 & 29700 & 29700 \\
0 & 100 & N & C2 & 87.89 & 95.81 & 29.32 & 75.77 & 74.65 & 85.50 & 29700 & 29700 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 29700 & 29700 \\
100 & 100 & GT & C1 & 87.33 & 95.87 & 24.08 & 74.66 & 73.36 & 84.76 & 29700 & 29700 \\
100 & 100 & GT & C2 & 90.59 & 96.42 & 27.59 & 76.87 & 74.99 & 85.80 & 29700 & 29700 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 99.85 & 100.00 & 47.41 & 84.00 & 82.72 & 91.01 & 29700 & 29700 \\
100 & 100 & N & C1 & 87.06 & 95.86 & 23.86 & 74.65 & 73.31 & 84.72 & 29700 & 29700 \\
100 & 100 & N & C2 & 89.89 & 96.39 & 25.99 & 76.05 & 74.44 & 85.51 & 29700 & 29700 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_vkitti-eval_depth.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, matched-training comparison. Depth is median-aligned per frame. U denotes unprovided depth views. ATE uses Sim(3) alignment and is expressed in the processed ground-truth units. nD and nU count eligible depth frames. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-vkitti-eval-depth}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrr@{}}
\toprule
D & C & Pose & Model & AbsRel$\downarrow$ & $\delta_1\uparrow$ & AbsRel-U$\downarrow$ & $\delta_{1,U}\uparrow$ & ATE-Sim(3)$\downarrow$ & $n_D$ & $n_U$ \\
\midrule
0 & 0 & -- & C1 & 0.080 & \textbf{92.15} & 0.080 & \textbf{92.15} & 5.40e-02 & 700 & 700 \\
0 & 0 & -- & C2 & 0.080 & 92.09 & 0.080 & 92.09 & \textbf{5.16e-02} & 700 & 700 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 0.071 & \textbf{93.37} & 0.077 & \textbf{92.59} & \textbf{5.39e-02} & 700 & 490 \\
30 & 0 & -- & C2 & 0.071 & 93.33 & 0.077 & 92.53 & 5.55e-02 & 700 & 490 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & 0.067 & \textbf{93.95} & 0.077 & \textbf{92.66} & \textbf{1.01e-01} & 700 & 350 \\
50 & 0 & -- & C2 & \textbf{0.066} & 93.93 & 0.077 & 92.61 & 1.73e-01 & 700 & 350 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 0.062 & \textbf{94.51} & 0.077 & \textbf{92.64} & 1.76e-01 & 700 & 210 \\
70 & 0 & -- & C2 & 0.062 & 94.49 & \textbf{0.076} & 92.60 & \textbf{1.62e-01} & 700 & 210 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & 0.056 & 95.39 & -- & -- & \textbf{4.22e-01} & 700 & 0 \\
100 & 0 & -- & C2 & \textbf{0.055} & 95.39 & -- & -- & 5.74e-01 & 700 & 0 \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 0.080 & \textbf{92.22} & 0.080 & \textbf{92.22} & \textbf{5.08e-02} & 700 & 700 \\
0 & 30 & GT & C2 & \textbf{0.079} & 92.16 & \textbf{0.079} & 92.16 & 5.84e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 0.080 & \textbf{92.22} & 0.080 & \textbf{92.22} & \textbf{5.18e-02} & 700 & 700 \\
0 & 50 & GT & C2 & \textbf{0.079} & 92.17 & \textbf{0.079} & 92.17 & 5.70e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 0.080 & \textbf{92.23} & 0.080 & \textbf{92.23} & \textbf{4.88e-02} & 700 & 700 \\
0 & 70 & GT & C2 & \textbf{0.079} & 92.17 & \textbf{0.079} & 92.17 & 5.75e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 0.080 & \textbf{92.23} & 0.080 & \textbf{92.23} & 3.75e-02 & 700 & 700 \\
0 & 100 & GT & C2 & \textbf{0.079} & 92.17 & \textbf{0.079} & 92.17 & \textbf{1.93e-02} & 700 & 700 \\
\addlinespace[1pt]
0 & 30 & N & C1 & 0.080 & \textbf{92.22} & 0.080 & \textbf{92.22} & \textbf{5.08e-02} & 700 & 700 \\
0 & 30 & N & C2 & \textbf{0.079} & 92.16 & \textbf{0.079} & 92.16 & 5.84e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 50 & N & C1 & 0.080 & \textbf{92.22} & 0.080 & \textbf{92.22} & \textbf{5.19e-02} & 700 & 700 \\
0 & 50 & N & C2 & \textbf{0.079} & 92.17 & \textbf{0.079} & 92.17 & 5.70e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 0.080 & \textbf{92.23} & 0.080 & \textbf{92.23} & \textbf{4.90e-02} & 700 & 700 \\
0 & 70 & N & C2 & \textbf{0.079} & 92.17 & \textbf{0.079} & 92.17 & 5.76e-02 & 700 & 700 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 0.080 & \textbf{92.23} & 0.080 & \textbf{92.23} & 3.77e-02 & 700 & 700 \\
0 & 100 & N & C2 & \textbf{0.079} & 92.17 & \textbf{0.079} & 92.17 & \textbf{2.28e-02} & 700 & 700 \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 0.056 & 95.40 & -- & -- & 3.72e-02 & 700 & 0 \\
100 & 100 & GT & C2 & \textbf{0.055} & 95.40 & -- & -- & \textbf{1.99e-02} & 700 & 0 \\
\addlinespace[1pt]
100 & 100 & N & C1 & 0.056 & 95.40 & -- & -- & 3.74e-02 & 700 & 0 \\
100 & 100 & N & C2 & \textbf{0.055} & 95.40 & -- & -- & \textbf{2.38e-02} & 700 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_vkitti-eval_directed.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, matched-training comparison. T-dir and A-dir use direction-sensitive translation errors. Thresholds are in degrees. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-vkitti-eval-directed}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrr@{}}
\toprule
D & C & Pose & Model & T-dir@2$\uparrow$ & T-dir@5$\uparrow$ & T-dir@15$\uparrow$ & A-dir@15$\uparrow$ & A-dir@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & \textbf{97.87} & 99.65 & 99.81 & \textbf{98.54} & \textbf{99.21} \\
0 & 0 & -- & C2 & 96.98 & \textbf{99.68} & \textbf{99.84} & 98.43 & 99.15 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & \textbf{96.92} & 99.65 & 99.84 & \textbf{98.40} & \textbf{99.14} \\
30 & 0 & -- & C2 & 95.46 & \textbf{99.68} & 99.84 & 98.17 & 99.01 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & \textbf{95.75} & \textbf{99.40} & \textbf{99.75} & \textbf{97.97} & \textbf{98.88} \\
50 & 0 & -- & C2 & 93.97 & 99.14 & 99.59 & 97.42 & 98.52 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & \textbf{95.84} & \textbf{99.08} & \textbf{99.62} & \textbf{97.80} & \textbf{98.75} \\
70 & 0 & -- & C2 & 94.29 & 98.98 & 99.59 & 97.50 & 98.61 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & \textbf{95.75} & \textbf{97.90} & \textbf{98.54} & \textbf{96.83} & \textbf{97.75} \\
100 & 0 & -- & C2 & 94.22 & 97.71 & 98.25 & 96.39 & 97.41 \\
\addlinespace[1pt]
0 & 30 & GT & C1 & \textbf{99.05} & 99.65 & \textbf{99.81} & \textbf{99.02} & \textbf{99.45} \\
0 & 30 & GT & C2 & 98.10 & \textbf{99.68} & 99.78 & 98.86 & 99.33 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & \textbf{98.95} & \textbf{99.68} & \textbf{99.81} & \textbf{98.97} & \textbf{99.43} \\
0 & 50 & GT & C2 & 97.75 & 99.56 & 99.78 & 98.74 & 99.27 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & \textbf{97.68} & \textbf{99.33} & \textbf{99.84} & \textbf{98.75} & \textbf{99.32} \\
0 & 70 & GT & C2 & 97.14 & 99.02 & 99.56 & 98.35 & 99.05 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 99.27 & 99.71 & 99.84 & 99.40 & 99.66 \\
0 & 100 & GT & C2 & \textbf{99.59} & \textbf{99.81} & \textbf{99.94} & \textbf{99.76} & \textbf{99.87} \\
\addlinespace[1pt]
0 & 30 & N & C1 & \textbf{99.08} & 99.65 & \textbf{99.81} & \textbf{99.02} & \textbf{99.45} \\
0 & 30 & N & C2 & 98.06 & \textbf{99.68} & 99.78 & 98.85 & 99.33 \\
\addlinespace[1pt]
0 & 50 & N & C1 & \textbf{98.92} & \textbf{99.68} & \textbf{99.81} & \textbf{98.98} & \textbf{99.43} \\
0 & 50 & N & C2 & 97.78 & 99.56 & 99.78 & 98.74 & 99.27 \\
\addlinespace[1pt]
0 & 70 & N & C1 & \textbf{97.59} & \textbf{99.27} & \textbf{99.84} & \textbf{98.74} & \textbf{99.31} \\
0 & 70 & N & C2 & 97.21 & 99.02 & 99.56 & 98.35 & 99.05 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 99.24 & 99.68 & 99.84 & 99.39 & 99.66 \\
0 & 100 & N & C2 & \textbf{99.59} & \textbf{99.81} & \textbf{99.94} & \textbf{99.72} & \textbf{99.85} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 98.73 & 99.75 & 99.87 & 99.17 & 99.54 \\
100 & 100 & GT & C2 & \textbf{99.27} & \textbf{99.81} & \textbf{99.94} & \textbf{99.64} & \textbf{99.79} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 98.63 & 99.75 & 99.87 & 99.13 & 99.52 \\
100 & 100 & N & C2 & \textbf{99.27} & \textbf{99.78} & \textbf{99.94} & \textbf{99.60} & \textbf{99.77} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_vkitti-eval_pose.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, matched-training comparison. R, T and A denote RRA, RTA and AUC. Angular thresholds are in degrees; T and A use sign-free translation errors. Bold marks the better displayed score within each matched pair.}
\label{tab:trained-vkitti-eval-pose}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & R@15$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & T@15$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ \\
\midrule
0 & 0 & -- & C1 & 100.00 & 100.00 & 100.00 & \textbf{97.87} & 99.65 & 99.81 & \textbf{98.54} & \textbf{99.21} \\
0 & 0 & -- & C2 & 100.00 & 100.00 & 100.00 & 96.98 & \textbf{99.68} & \textbf{99.84} & 98.43 & 99.15 \\
\addlinespace[1pt]
30 & 0 & -- & C1 & 100.00 & 100.00 & 100.00 & \textbf{96.92} & 99.65 & 99.84 & \textbf{98.40} & \textbf{99.14} \\
30 & 0 & -- & C2 & 100.00 & 100.00 & 100.00 & 95.46 & \textbf{99.68} & 99.84 & 98.17 & 99.01 \\
\addlinespace[1pt]
50 & 0 & -- & C1 & \textbf{99.43} & 100.00 & 100.00 & \textbf{95.75} & \textbf{99.40} & \textbf{99.75} & \textbf{97.97} & \textbf{98.89} \\
50 & 0 & -- & C2 & 98.89 & 100.00 & 100.00 & 93.97 & 99.14 & 99.65 & 97.46 & 98.57 \\
\addlinespace[1pt]
70 & 0 & -- & C1 & 99.30 & 100.00 & 100.00 & \textbf{95.84} & \textbf{99.08} & \textbf{99.65} & \textbf{97.81} & \textbf{98.78} \\
70 & 0 & -- & C2 & \textbf{99.33} & 100.00 & 100.00 & 94.29 & 98.98 & 99.62 & 97.51 & 98.63 \\
\addlinespace[1pt]
100 & 0 & -- & C1 & \textbf{98.95} & 100.00 & 100.00 & \textbf{96.16} & 98.54 & 99.24 & \textbf{97.38} & 98.44 \\
100 & 0 & -- & C2 & 98.89 & 100.00 & 100.00 & 94.57 & \textbf{98.79} & \textbf{99.43} & 97.35 & \textbf{98.47} \\
\addlinespace[1pt]
0 & 30 & GT & C1 & 100.00 & 100.00 & 100.00 & \textbf{99.05} & 99.65 & \textbf{99.81} & \textbf{99.02} & \textbf{99.45} \\
0 & 30 & GT & C2 & 100.00 & 100.00 & 100.00 & 98.10 & \textbf{99.68} & 99.78 & 98.86 & 99.33 \\
\addlinespace[1pt]
0 & 50 & GT & C1 & 100.00 & 100.00 & 100.00 & \textbf{98.95} & \textbf{99.68} & \textbf{99.81} & \textbf{98.97} & \textbf{99.43} \\
0 & 50 & GT & C2 & 100.00 & 100.00 & 100.00 & 97.75 & 99.56 & 99.78 & 98.74 & 99.27 \\
\addlinespace[1pt]
0 & 70 & GT & C1 & 100.00 & 100.00 & 100.00 & \textbf{97.68} & \textbf{99.33} & \textbf{99.84} & \textbf{98.75} & \textbf{99.32} \\
0 & 70 & GT & C2 & 100.00 & 100.00 & 100.00 & 97.14 & 99.02 & 99.56 & 98.35 & 99.05 \\
\addlinespace[1pt]
0 & 100 & GT & C1 & 100.00 & 100.00 & 100.00 & 99.27 & 99.71 & 99.84 & 99.40 & 99.66 \\
0 & 100 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{99.59} & \textbf{99.81} & \textbf{99.94} & \textbf{99.76} & \textbf{99.87} \\
\addlinespace[1pt]
0 & 30 & N & C1 & 100.00 & 100.00 & 100.00 & \textbf{99.08} & 99.65 & \textbf{99.81} & \textbf{99.02} & \textbf{99.45} \\
0 & 30 & N & C2 & 100.00 & 100.00 & 100.00 & 98.06 & \textbf{99.68} & 99.78 & 98.85 & 99.33 \\
\addlinespace[1pt]
0 & 50 & N & C1 & 100.00 & 100.00 & 100.00 & \textbf{98.92} & \textbf{99.68} & \textbf{99.81} & \textbf{98.98} & \textbf{99.43} \\
0 & 50 & N & C2 & 100.00 & 100.00 & 100.00 & 97.78 & 99.56 & 99.78 & 98.74 & 99.27 \\
\addlinespace[1pt]
0 & 70 & N & C1 & 100.00 & 100.00 & 100.00 & \textbf{97.59} & \textbf{99.27} & \textbf{99.84} & \textbf{98.74} & \textbf{99.31} \\
0 & 70 & N & C2 & 100.00 & 100.00 & 100.00 & 97.21 & 99.02 & 99.56 & 98.35 & 99.05 \\
\addlinespace[1pt]
0 & 100 & N & C1 & 100.00 & 100.00 & 100.00 & 99.24 & 99.68 & 99.84 & 99.39 & 99.66 \\
0 & 100 & N & C2 & 100.00 & 100.00 & 100.00 & \textbf{99.59} & \textbf{99.81} & \textbf{99.94} & \textbf{99.72} & \textbf{99.85} \\
\addlinespace[1pt]
100 & 100 & GT & C1 & 100.00 & 100.00 & 100.00 & 98.73 & 99.75 & 99.87 & 99.17 & 99.54 \\
100 & 100 & GT & C2 & 100.00 & 100.00 & 100.00 & \textbf{99.27} & \textbf{99.81} & \textbf{99.94} & \textbf{99.64} & \textbf{99.79} \\
\addlinespace[1pt]
100 & 100 & N & C1 & 100.00 & 100.00 & 100.00 & 98.63 & 99.75 & 99.87 & 99.13 & 99.52 \\
100 & 100 & N & C2 & 100.00 & 100.00 & 100.00 & \textbf{99.27} & \textbf{99.78} & \textbf{99.94} & \textbf{99.60} & \textbf{99.77} \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> tables/generated/trained_vkitti-eval_retention.tex <==
\begin{table}[tbp]
\centering
\caption{Virtual KITTI 2, prior retention on provided--provided pairs. All three rows within an input condition use the same eligible pair support. R, T and A denote RRA, sign-free RTA and AUC.}
\label{tab:trained-vkitti-eval-retention}
\begingroup
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrclrrrrrrrr@{}}
\toprule
D & C & Pose & Model & R@2$\uparrow$ & R@5$\uparrow$ & T@2$\uparrow$ & T@5$\uparrow$ & A@15$\uparrow$ & A@30$\uparrow$ & $n_R$ & $n_T$ \\
\midrule
0 & 30 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 210 & 210 \\
0 & 30 & GT & C1 & 100.00 & 100.00 & 99.52 & 100.00 & 99.24 & 99.62 & 210 & 210 \\
0 & 30 & GT & C2 & 100.00 & 100.00 & 99.05 & 100.00 & 99.24 & 99.62 & 210 & 210 \\
\addlinespace[1pt]
0 & 50 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 700 & 700 \\
0 & 50 & GT & C1 & 100.00 & 100.00 & 100.00 & 100.00 & 99.75 & 99.88 & 700 & 700 \\
0 & 50 & GT & C2 & 100.00 & 100.00 & 100.00 & 100.00 & 99.80 & 99.90 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 1470 & 1470 \\
0 & 70 & GT & C1 & 100.00 & 100.00 & 99.93 & 100.00 & 99.75 & 99.87 & 1470 & 1470 \\
0 & 70 & GT & C2 & 100.00 & 100.00 & 100.00 & 100.00 & 99.85 & 99.93 & 1470 & 1470 \\
\addlinespace[1pt]
0 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 3150 & 3150 \\
0 & 100 & GT & C1 & 100.00 & 100.00 & 99.27 & 99.71 & 99.40 & 99.66 & 3150 & 3150 \\
0 & 100 & GT & C2 & 100.00 & 100.00 & 99.59 & 99.81 & 99.76 & 99.87 & 3150 & 3150 \\
\addlinespace[1pt]
0 & 30 & N & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 99.84 & 99.92 & 210 & 210 \\
0 & 30 & N & C1 & 100.00 & 100.00 & 99.52 & 100.00 & 99.11 & 99.56 & 210 & 210 \\
0 & 30 & N & C2 & 100.00 & 100.00 & 99.05 & 100.00 & 99.21 & 99.60 & 210 & 210 \\
\addlinespace[1pt]
0 & 50 & N & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 99.93 & 99.97 & 700 & 700 \\
0 & 50 & N & C1 & 100.00 & 100.00 & 100.00 & 100.00 & 99.77 & 99.89 & 700 & 700 \\
0 & 50 & N & C2 & 100.00 & 100.00 & 100.00 & 100.00 & 99.79 & 99.90 & 700 & 700 \\
\addlinespace[1pt]
0 & 70 & N & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 99.95 & 99.98 & 1470 & 1470 \\
0 & 70 & N & C1 & 100.00 & 100.00 & 100.00 & 100.00 & 99.77 & 99.89 & 1470 & 1470 \\
0 & 70 & N & C2 & 100.00 & 100.00 & 100.00 & 100.00 & 99.83 & 99.91 & 1470 & 1470 \\
\addlinespace[1pt]
0 & 100 & N & Prior & 100.00 & 100.00 & 99.78 & 99.90 & 99.89 & 99.95 & 3150 & 3150 \\
0 & 100 & N & C1 & 100.00 & 100.00 & 99.24 & 99.68 & 99.39 & 99.66 & 3150 & 3150 \\
0 & 100 & N & C2 & 100.00 & 100.00 & 99.59 & 99.81 & 99.72 & 99.85 & 3150 & 3150 \\
\addlinespace[1pt]
100 & 100 & GT & Prior & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 3150 & 3150 \\
100 & 100 & GT & C1 & 100.00 & 100.00 & 98.73 & 99.75 & 99.17 & 99.54 & 3150 & 3150 \\
100 & 100 & GT & C2 & 100.00 & 100.00 & 99.27 & 99.81 & 99.64 & 99.79 & 3150 & 3150 \\
\addlinespace[1pt]
100 & 100 & N & Prior & 100.00 & 100.00 & 99.78 & 99.90 & 99.89 & 99.95 & 3150 & 3150 \\
100 & 100 & N & C1 & 100.00 & 100.00 & 98.63 & 99.75 & 99.13 & 99.52 & 3150 & 3150 \\
100 & 100 & N & C2 & 100.00 & 100.00 & 99.27 & 99.78 & 99.60 & 99.77 & 3150 & 3150 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\endgroup
\end{table}

